DisCo RL: Distribution-Conditioned Reinforcement Learning for General-Purpose Policies

Can we use reinforcement learning to learn general-purpose policies that can perform a wide range of different tasks, resulting in flexible and reusable skills? Contextual policies provide this capability in principle, but the representation of the context determines the degree of generalization and expressivity. Categorical contexts preclude generalization to entirely new tasks. Goal-conditioned policies may enable some generalization, but cannot capture all tasks that might be desired. In this paper, we propose goal distributions as a general and broadly applicable task representation suitable for contextual policies. Goal distributions are general in the sense that they can represent any state-based reward function when equipped with an appropriate distribution class, while the particular choice of distribution class allows us to trade off expressivity and learnability. We develop an off-policy algorithm called distribution-conditioned reinforcement learning (DisCo RL) to efficiently learn these policies. We evaluate DisCo RL on a variety of robot manipulation tasks and find that it significantly outperforms prior methods on tasks that require generalization to new goal distributions.

==> draft/2_introduction_short.tex <==
\section{Introduction}
Versatile, general-purpose robotic systems will require not only broad repertoires of behavioral skills, but also the faculties to quickly acquire new behaviors as demanded by their current situation and the needs of their users.
Reinforcement learning (RL) in principle enables autonomous acquisition of such skills. However, each skill must be learned individually at considerable cost in time and effort.
In this paper, we instead explore how general-purpose robotic policies can be acquired by conditioning policies on task representations.
This question has previously been investigated by learning \emph{goal-conditioned} or \emph{universal} policies, which take in not only the current state, but also some representation of a \emph{goal} state.
However, such a task representation cannot capture many of the behaviors we might actually want a versatile robotic system to perform, since it can only represent behaviors that involve reaching individual states.
For example, for a robot packing items into a box, the task is defined by the position of the items relative to the box, rather than their absolute locations in space, and therefore does not correspond to a single state configuration.
How can we parameterize a more general class of behaviors, so as to make it possible to acquire truly general-purpose policies that, if conditioned appropriately, could perform any desired task?


To make it possible to learn general-purpose policies that can perform any task, we instead consider conditioning a policy on a full \emph{distribution} over goal states.
Rather than reaching a specific state, a policy must learn to reach states that have high likelihood under the provided distribution, which may specify various covariance relationships (e.g., as shown in Figure~\ref{fig:gcdrl-intuition}, that the position of the items should covary with the position of the box).
In fact, we show that, because optimal policies are invariant to additive factors in reward functions, arbitrary goal distributions can represent \textit{any} state-dependent reward function, and therefore any task.
Choosing a specific distribution class provides a natural mechanism to control the expressivity of the policy.
We may choose a small distribution class to narrow the range of tasks and make learning easier, or we may choose a large distribution class to expand the expressiveness of the policy.



Our experiments demonstrate that distribution-conditioned policies can be trained efficiently by sharing data from a variety of tasks and relabeling the goal distribution parameters, where each distribution corresponds to a different task reward.
Lastly, while the distribution parameters can be provided manually to specify tasks, we also present two ways to infer these distribution parameters directly from data.


The main contribution of this paper is \METHOD, an algorithm for learning distribution-conditioned policies.
To learn efficiently, \METHOD uses off-policy training and a novel distribution relabeling scheme.
We evaluate on robot manipulation tasks in which a single policy must solve multiple tasks that cannot be expressed as reaching different goal states.
We find that conditioning the policies on goal distributions results in significantly faster learning than solving each task individually, enabling policies to acquire a broader range of tasks than goal-conditioned methods.


\begin{figure}[t]
    \centering
    \vspace{-0.05in}
    \includegraphics[width=0.75\linewidth]{figures/illustrative/fig1v62.pdf}
    \vspace{-0.5cm}
    \caption{
    We infer the distribution parameters $\gdparam$ from data and pass it to a \METHODADJ policy.
    Distribution-conditioned RL can express a broad range of tasks,
    from defining relationships between different state components (top)
    to more arbitrary behavior (bottom).
    }
    \label{fig:gcdrl-intuition}
    \vspace{-0.145in}
\end{figure}

==> draft/4_background_short.tex <==
\section{Background}\label{sec:background}
Reinforcement learning (RL) 
frames reward maximization in a Markov decision process (MDP), defined by the tuple $\gM = (\gS, \gA, r, p, p_{0}, \gamma )$~\citep{sutton1998rl}, where $\gS$ denotes the state space and $\mathcal{A}$ denotes the action space.
In each episode, the agent's initial state $\bs_0 \in \gS$ is
sampled from an initial state distribution $\bs_0 \sim p_0(\bs_0)$, the agent chooses an action $\ba \in \mathcal{A}$ according to a stochastic policy $\ba_t \sim \pi( \cdot | \bs_t)$, and the next state is generated from the state transition dynamics $\bs_{t+1} \sim p(\cdot \mid \bs_t, \ba_t)$.
We will use $\tau$ to denote a trajectory sequence $(\bs_0, \ba_0, \bs_1, \dots)$ and denote sampling as \mbox{$\tau \sim \pi$} since we assume a fixed initial state and dynamics distribution.
The objective of an agent is to maximize the sum of discounted rewards,
% \begin{align}\label{eq:standard-mdp}
    $\E_{\tau \sim \pi}\left[\sum_{t=1}^\infty \gamma^t r(\bs_t, \ba_t)\right]$.
% \end{align}

\noindent \textbf{Off-policy, temporal-difference algorithms.}
Our method can be used with any off-policy temporal-difference (TD) learning algorithm.
TD-learning algorithms only need $(\bs_{t}, \ba_{t}, r_{t}, \bs_{t+1})$ tuples to train a policy, where $\ba_{t}$ is an action taken from state $\bs_{t}$, and where $r_{t}$ and $\bs_{t+1}$ are the resulting reward and next state, respectively, sampled from the environment.
Importantly, these tuples can be collected by any policy, making it an off-policy algorithm.
These tuples are typically sampled from a replay buffer $\replay$, which consists of tuples generated by all previous environment interactions.



==> draft/5_method_short.tex <==
\section{\METHODLONG}
In this section, we show how conditioning policies on a goal distribution results in a MDP that can capture any set of reward functions.
Each distribution represents a different reward function, and so choosing a distribution class provides a natural mechanism to choose the expressivity of the contextual policy.
We then present \methodlong (\METHOD), an off-policy algorithm for training policies conditioned on parametric representation of distributions, and discuss the specific representation that we use.

\subsection{Generality of Goal Distributions}
We assume that the goal distribution is in a parametric family, with parameter space $\gdspace$, and augment the MDP state space with the goal distribution, as in $\gS' = \gS \times \gdspace$.
At the beginning of each episode, a parameter $\gdparam \in \gdspace$ is sampled from some parameter distribution $p_\gdparam$.
The parameter $\gdparam$ defines the goal distribution \mbox{$p_g(\bs ; \gdparam): \gS \mapsto \R_+$} over the state space.
The policy is conditioned on this parameter, and is given by $\pi(\cdot \mid \bs, \gdparam)$.
The objective of a distribution-conditioned (\METHODADJ) policy is to reach states that have high log-likelihood under the goal distribution, which can be expressed as
\begin{align}\label{eq:gdc-objective}
    \max_\pi \E_{\tau \sim \pi(\cdot \mid \bs, \gdparam)}\left[\sum_t \gamma^t \log p_g(\bs_t; \gdparam)\right].
    %%SL.7.26: Equation is better now, but maybe explicitly condition pi on omega?
\end{align}
This formulation can express arbitrarily complex distributions and tasks, as we illustrate in \autoref{fig:gcdrl-intuition}. More formally:
\begin{remark}
Any reward maximization problem
can be equivalently written as maximizing the log-likelihood under a goal distribution (\autoref{eq:gdc-objective}), up to a constant factor.
\end{remark}
This statement is true because, for any reward function of the form $r(\bs)$, we can define a distribution \mbox{$p_g(\bs) \propto e^{r(\bs)}$},
% \begin{align*}
%     p_g(s) = \frac{e^{r(s)}}{\int_{s'} e^{r(s')} ds'},
% \end{align*}
from which we can conclude that maximizing $\log p_g(\bs)$ is equivalent to maximizing $r(\bs)$, up to the constant normalizing factor in the denominator.
If the reward function depends on the action, $r(\bs, \ba)$, we can modify the MDP and append the previous action to the state $\bar{\bs} = [\bs, \ba]$, reducing it to another MDP with a reward function of the form $r(\bar{\bs})$.

Of course, while any reward can be expressed as the log-likelihood of a goal distribution, a specific fixed parameterization $p_g(\bs ; \gdparam)$ may not by itself be able to express any reward.
In other words, choosing the distribution parameterization is equivalent to choosing the set of reward functions that the conditional policy can maximize.
As we discuss in the next section, we can trade-off expressivity and ease of learning by choosing an appropriate goal distribution family.

\subsection{Goal Distribution Parameterization}\label{sec:goal-distribution-parameterization}

Different distribution classes represent different types of reward functions.
To explore the different capabilities afforded by different distributions, we study three families of distributions.
\paragraph{Gaussian distribution}
A simple class of distributions is the family of multivariate Gaussian.
Given a state space in $\R^n$, the distribution parameters consists of two components, \mbox{$\gdparam = (\bmu, \Sigma)$}, where \mbox{$\bmu \in \R^n$} is the mean vector and \mbox{$\Sigma \in \R^{n \times n}$} is the covariance matrix.
When inferring the distribution parameters with data, we regularize the $\Sigma^{-1}$ matrix by thresholding absolute values below $\epsilon = 0.25$ to zero.
With these parameters, the reward from \autoref{eq:gdc-objective} is given by
% \begin{align}\label{eq:gaussian-log-prob-reward}
\mbox{$
    r(\bs; \omega) = -0.5 (\bs - \bmu)^T \Sigma^{-1} (\bs - \bmu),
$}
% \end{align}
where we have dropped constant terms that do not depend on the state $\bs$. % and added a square-root, which we found to perform better in practice.
This simple parameterization can express a large number of reward functions.
Using this parameterization, the weight of individual state dimensions depend on the values along the diagonal of the covariance matrix.
By using off-diagonal covariance values, this parameterization also captures the set of tasks in which state components need to covary, such as when the one object must be placed near another one, regardless of the exact location of those objects (see the top half of \autoref{fig:gcdrl-intuition}).
% In practice, we found that the reward
% \mbox{
% $
%     r(\bs; \omega) = -0.5 \sqrt{(\bs - \bmu)^T \Sigma^{-1} (\bs - \bmu)}
% $
% }
% with the square-root performed slight better, and so we used this reward.

\paragraph{Gaussian mixture model}
A more expressive class of distributions that we study is the Gaussian mixture model with 4 modes, which can represent multi-modal tasks.
\optional{
The parameters are the mean and covariance of each Gaussian and the weight assigned to each Gaussian distribution. The reward is given by the log-likelihood of a state.
}

\paragraph{Latent variable model}
To study an even more express class of distribution, we consider a class of distributions parameterized by neural networks.
Distributions parameterized by neural networks can be extremely expressive~\citep{dinh2016density, van2016conditional}, but distributions based on neural networks often have millions of parameters~\citep{dinh2016density, kingma2018glow}.

To obtain an expressive yet compact parameterization, we consider non-linear reparameterizations of the original state space.
Specifically, we model a distribution over the state space using a Gaussian variational auto-encoder (VAE)~\citep{kingma2014vae,rezende2014stochasticbackprop}.
Gaussian VAEs model a set of observations using a latent-variable model of the form
% \begin{align*}
\mbox{
$
    p(\bs) = \int_{\gZ} p(\bz) p_\decparam(\bs \mid \bz) d\bz,
$
}
% \end{align*}
where $\bz \in \gZ = \mathbb{R}^{d_z}$ are latent variables with dimension $d_z$.
The distribution $p_\decparam$ is a learned generative model or ``decoder'' and $p(z)$ is a standard multivariate Gaussian distribution in $\R^{d_z}$.
A Gaussian VAE also learns a posterior distribution or ``encoder'' that maps states $\bs$ onto Gaussian distributions in a latent space, given by $q_\encparam(\bz; \bs)$.
We refer readers to \citet{doersch2016tutorial} for a detailed explanation of VAEs.

Gaussian VAEs are explicitly trained so that Gaussian distributions in a latent space define distributions over the state space.
Therefore, we represent a distribution over the state space with the mean $\bmu_z \in \mathbb{R}^{d_z}$ and variances $\bsigma_z \in \mathbb{R}^{d_z}$ of a diagonal Gaussian distribution \emph{in the learned, latent space}, which we write as $\gN(\bz; \bmu_z, \bsigma_z)$.
In other words, the parameters $\gdparam = (\bmu_z, \bsigma_z )$ define the following distribution over the states:
\begin{align}\label{eq:non-linear-param}
    p_g(\bs; \omega) = \int_{\gZ} \gN (\bz ; \bmu_z, \bsigma_z) p_\decparam(\bs \mid \bz) d\bz,
\end{align}
where $p_\decparam(\bs \mid \bz)$ is the generative model from the VAE.
Because $\bz$ resides in a learned latent space, the set of reward functions that can be expressed with \Cref{eq:non-linear-param} includes arbitrary non-linear transformations of $\bs$.

\section{Learning Goal Distributions and Policies}\label{sec:goal-distribution-inference}
Given any of the distribution classes mentioned above, we now consider how to obtain a specific goal distribution parameter $\gdparam$ and train a policy to maximize \Cref{eq:gdc-objective}.
We start with obtaining goal distribution parameters $\gdparam$.
While a user can manually select the goal distribution parameters $\gdparam$, this requires a degree of user insight, which can be costly or practically impossible if using the latent representation in \Cref{eq:non-linear-param}.
We discuss two automated alternatives for obtaining the goal distribution parameters $\gdparam$.% in each case.

\subsection{Inferring Distributions from Examples}
\label{sec:infer-from-examples}
One simple and practical way to specify a goal distribution is to provide $K$ example observations $\{\bs_k\}_{k=1}^K$ in which the task is successfully completed.
This supervision can be easier to provide than full demonstrations, which not only specify the task but also must show how to solve the task through a sequence of states $(\bs_1, \bs_2, \dots)$ or states and actions $(\bs_1, \ba_1, \bs_2, \dots)$.
Given the example observations, we describe a way to infer the goal parameter based on the parameterization.

If $\gdparam$ represents the parameters of a distribution in the state space, we learn a goal distribution via maximum likelihood estimation (MLE), as in
\begin{align}\label{eq:state-gd-inference}
    \gdparam^* = \argmax_{\gdparam \in \gdspace} \sum_{k=1}^K \log p_g(\bs_k; \gdparam),
\end{align}
and condition the policy on the resulting parameter $\gdparam^*$.
If $\gdparam$ represents the parameters of a distribution in the latent space, we need a Gaussian distribution in the latent space that places high likelihood on all of the states in $\dtask$.
We obtain such a distribution by finding a latent distribution that minimizes the KL divergence to the mixture of posteriors $\frac{1}{K} \sum_k q_\encparam(\gdparam ; \bs_k)$.
Specifically, we solve the problem
\begin{align}\label{eq:latent-space-gd-inference}
    \gdparam^* = \argmin_{\gdparam \in \gdspace} \DKL{
    \frac{1}{K} \sum_k q_\encparam(\bz ; \bs_k)
    }{p(\bz; \gdparam)},
\end{align}
where $\gdspace$ is the set of all means and diagonal covariance matrices in $\R^{d_z}$.
The solution to \Cref{eq:latent-space-gd-inference} can be computed in closed form using moment matching~\citep{minka2001expectation}.



\subsection{Dynamically Generating Distributions via Conditioning}
\label{sec:infer-conditional}
We also study a different use case for training a \METHODADJ policy:
automatically decomposing long-horizon tasks into sub-tasks.
Many complex tasks lend themselves to such a decomposition, and learning each of these sub-tasks can be significantly faster than directly solving the main task.
For example, a robot that must arrange a table can divide this task into placing one object to a desired location before moving on to the next object.
To automatically decompose a task, we need to convert a ``final task,'' represented as $\taskparam$, into $M$ different sub-tasks, where $M$ is the number of sub-tasks needed to accomplish the final task.
Moreover, rather than training a separate policy for each sub-task, we would like to train a single policy that can accomplish all of these sub-tasks.
How can we convert a task parameter $\taskparam$ into different sub-tasks, all of which can be accomplished by a single policy?

\begin{wrapfigure}{r}{0.6\textwidth}
    \vspace{-0.5cm}
    \centering
    \includegraphics[width=\linewidth]{figures/illustrative/fig2_v6.pdf}
    \caption{
    % (Left)
    A robot must arrange objects into a configuration $\bs_f$ that changes from episode to episode.
    This task consists of multiple sub-tasks, such as first moving the red object to the correct location.
    Given a final state $\bs_f$, there exists a distribution of intermediate states $\bs$ in which the first sub-task is completed.
    % (Right)
    We use pairs of states $\bs, \bs_f$ to learn a conditional distribution that defines the first sub-task given the final task, \mbox{$p(\bs \mid \bs_f)$}.}
    \label{fig:conditional-distribution-visualization}
    \vspace{-0.8cm}
\end{wrapfigure}


We can address this question by training a \METHODADJ policy.
A task represented by parameters $\taskparam$ can be decomposed into a sequence of sub-tasks, each of which in turn is represented by a goal distribution.
We accomplish this by learning \textit{conditional distributions}, $p_g^i(\bs \mid \taskparam)$:
conditioned on some final task $\taskparam$, the conditional distribution $p_g^i(\bs \mid \taskparam)$ is a distribution over desired states for sub-task $i$.

To obtain a conditional distribution $p_g^i(\bs \mid \taskparam)$ for sub-task $i$, we assume access to tuples \mbox{$\dtask ^i = \{(\bs^{(k)}, \taskparam^{(k)})\}_{k=1}^K$}, where $\bs^{(k)}$ is an example state in which sub-task $i$ is accomplished for solving task $\taskparam^{(k)}$.
See \Cref{fig:conditional-distribution-visualization} for a visualization.
Our experiments test the setting where final tasks are represented by a final state $\bs_f$ that we want the robot to reach, meaning that \mbox{$\taskparam = \bs_f$}.
We note that one can train a goal-conditioned policy to reach this final state $\bs_f$ directly, but, as we will discuss in \Cref{sec:experiments}, this decomposition significantly accelerates learning by exploiting access to the pairs of states.

For each $i$, and dropping the dependence on $i$ for clarify, we learn a conditional distribution, by fitting a joint Gaussian distribution, denoted by \mbox{$p_{\bS, \bS_f}(\bs, \bs_f; \bmu, \Sigma)$}, to these pairs of states using MLE, as in
\begin{align}\label{eq:learn-joint-distrib}
    \bmu^*, \Sigma^* = \argmax_{\mu, \Sigma} \sum_{k=1}^K \log p_{\bS, \bS_f}(\bs^{(k)}, \bs_f^{(k)}; \bmu, \Sigma).
    % \bmu^*, \Sigma^* = \argmax_{\mu, \Sigma} \sum_{k=1}^K \log p_{\bS, \bS_f}(\bs^{(k)}, \bs_f^{(k)};
    % \begin{bmatrix}
    % \mu_1\\
    % \mu_2
    % \end{bmatrix}
    % ,
    % \begin{bmatrix}
    % \Sigma_{11} & \Sigma_{12}\\
    % \Sigma_{21} & \Sigma_{22}
    % \end{bmatrix}
    % ).
\end{align}
This procedure requires up-front supervision for each sub-task during training time, but at test time, given a desired final state $\bs_f$, 
% we can compute the conditional goal distribution
% \begin{align}
%     p_g(\bs | \taskparam = \bs_f) = p_{\bS | \bS_f}(\bs \mid \bs_f; \mu^*, \Sigma^*)
% \end{align}
% in closed form.\footnote{
% Given the Gaussian parameters $\bmu^* = \begin{bmatrix}\mu_1\\ \mu_2\end{bmatrix}$
% and $\Sigma^* = \begin{bmatrix}\Sigma_{11} & \Sigma_{12} \\ \Sigma_{21} & \Sigma_{22} \end{bmatrix}$, the parameters of a conditional distribution over the state $\bs$ conditioned on a final goal state $\bs_f$ are
% $\bar \mu = \mu_1 + \sigma_{12} \sigma_{22}^{-1}(\bs_f - \mu_2)$
% and
% $\bar \sigma = \sigma_{11} - \sigma_{12} \sigma_{22}^{-1} \sigma_{21}$.
% }
we compute the parameters of the Gaussian conditional distribution $p_g(\bs \mid \bs_f; \mu^*, \Sigma^*)$ in closed form. Specifically, the conditional parameters are given by
% \begin{align}\label{eq:conditional-params}
% \bar \mu = \mu_1 + \Sigma_{12} \Sigma_{22}^{-1}(\bs_f - \mu_2)\quad
% \bar \Sigma = \Sigma_{11} - \Sigma_{12} \Sigma_{22}^{-1} \Sigma_{21},
% \end{align}
\begin{equation}
  \label{eq:conditional-params}
  \begin{aligned}
\bar \mu &= \mu_1 + \Sigma_{12} \Sigma_{22}^{-1}(\bs_f - \mu_2)\\
\bar \Sigma &= \Sigma_{11} - \Sigma_{12} \Sigma_{22}^{-1} \Sigma_{21},
  \end{aligned}
\end{equation}
where $\mu_1$ and $\mu_2$ represents the first and second half of $\mu^*$, and similarly for the covariance terms.
To summarize, we learn $\mu^*$ and $\Sigma^*$ with \Cref{eq:learn-joint-distrib} and then use \Cref{eq:conditional-params} to automatically transform a final task $\taskparam = \bs_f$ into a goal distribution $\gdparam = (\bar \mu, \bar \Sigma)$ which we give to a \METHODADJ policy.
Having presented two ways to obtain distributions, we now turn to learning \METHOD policies.



\subsection{Learning Distribution-Conditioned Policies}\label{sec:learning-disco-policies}
In this section, we discuss how to optimize \autoref{eq:gdc-objective} using an off-policy TD algorithm.
As discussed in \autoref{sec:background}, TD algorithms require tuples of state, action, next state, and reward, denoted by $(\bs_{t}, \ba_{t}, r_{t}, \bs_{t+1})$.
To collect this data, we condition a policy on a goal distribution parameter $\gdparam$, collect a trajectory with the policy \mbox{$\tau = [\bs_0, \ba_0, \cdots]$}, and then store the trajectory and distribution parameter into a replay buffer~\citep{mnih2015human}, denoted as $\gR$.
We then sample data from this replay buffer to train our policy using an off-policy TD algorithm.
% In our experiments,
We use soft actor-critic as our RL algorithm~\citep{haarnoja2018sac}, though in theory any off-policy algorithm could be used.
Because TD algorithms are off-policy, we propose to reuse data collected by a policy conditioned on one goal distribution $\gdparam$ to learn about how a policy should behave under another goal distribution $\gdparam'$.
In particular, given a state $\bs$ sampled from a policy that was conditioned on some goal distribution parameters $\gdparam$, we occasionally relabel the goal distribution with an alternative goal distribution \mbox{$\gdparam' = \RS(\bs, \gdparam)$} for training, where $\RS$ is some relabeling strategy.
For relabeling, given a state $\bs$ and existing parameters $\gdparam = (\mu, \Sigma)$, we would like to provide a strong learning signal by creating a distribution parameter that gives high reward to an achieved state.
We used a simple strategy that we found worked well:
we replace the mean with the state vector $\bs$ and randomly re-sampling the covariance from the set of observed covariances as in $\RS(\bs, (\mu, \Sigma)) =  (\bs, \Sigma')$, where $\Sigma'$ is sampled uniformly from the replay buffer.
This relabeling is similar to relabeling methods used in goal-conditioned reinforcement learning~\citep{kaelbling1993goals,andrychowicz2017her,rauber2017hindsight,pong2018tdm,nachum2018hiro,plappert2018multigoal,nair2018rig,eysenbach2020rewriting}, but applied to goal distributions rather than individual goal states.

% \vspace{0.3cm}
\setlength{\textfloatsep}{6pt}
\begin{algorithm}[t]
\caption{\blue{(Conditional)} Distribution-Conditioned RL}
\label{algo:disco}
\begin{algorithmic}[1]
\REQUIRE Policy $\pi_\ppi$, $Q$-function $Q_\pq$, TD algorithm $\gA$, relabeling strategy $\RS$, exploration parameter distribution $p_\gdparam$, replay buffer $\gR$.
% \STATE \red{(if unconditional)} compute $\gdparam$ using \Cref{eq:state-gd-inference,eq:latent-space-gd-inference}.
% \STATE Compute $\gdparam$ using \Cref{eq:state-gd-inference} or \Cref{eq:latent-space-gd-inference}.
\STATE Compute $\gdparam$ using Equation (4) or (5) \blue{(if unconditional)}.
\FOR{$0, \dots, N_\text{episode}-1$ episodes}
    % \STATE \red{Sample task $\taskparam$ and compute $\gdparam = \text{param}[p(\bs \mid \taskparam)]$.}\footnote{The notation \texttt{params}$[p]$ indicates computing the parameters of the distribution $p$}
    % \STATE \red{Sample task $\taskparam$ and compute $\gdparam = \text{param}[p(\bs \mid \taskparam)]$.}\footnote{The notation \texttt{params}$[p]$ indicates computing the parameters of the distribution $p$}
    \STATE \blue{Sample $\bs_f$ and compute $\gdparam$ with \Cref{eq:conditional-params}.}
    % \STATE Sample state \mbox{$\bs_0 \sim p_0$} and parameter \mbox{$\gdparam \sim p_\gdparam(\cdot \red{\mid \taskparam})$}
    % \STATE Sample state \mbox{$\bs_0 \sim p_0$} and parameter \mbox{$\gdparam \sim p_\gdparam(\cdot \red{\mid \taskparam})$}
    % \STATE Sample state \mbox{$\bs_0 \sim p_0$} and parameter \mbox{$\gdparam \sim p_\gdparam(\cdot \red{\mid \taskparam})$}
    % \STATE Sample initial state $\bs_0 \sim p_0$.
    \STATE Sample trajectory from environment $\tau \sim \pi(\cdot | \bs; \gdparam)$ and store tuple $(\tau, \gdparam)$ in replay buffer $\gR$.
    % \FOR{$t=0, \dots, H-1$ steps}
    %     \STATE Sample action $\ba_t \sim \pi_\ppi(\cdot \mid \bs_t, \gdparam)$ and next state $\bs_{t+1} \sim p(\cdot \mid \bs_t, \ba_t)$.
    %     \STATE Store $(\bs_t, \ba_t, \bs_{t+1}, \gdparam)$ into replay buffer $\gR$.
    % \ENDFOR
    \FOR{$0, \dots,  N_\text{updates}-1$ steps}
        \STATE Sample trajectory and parameter $(\tau, \gdparam) \sim \gR$.
        % \STATE Sample two time steps $t, h \in \{0, \dots, \text{length}(\tau)\}$, where $t < h$.
        \STATE Sample transition tuple $(\bs_t, \ba_t, \bs_{t+1})$ and a future state $\bs_h$ from $\tau$, where $t < h$.
        \STATE With probability $p_\text{relabel}$, relabel $\gdparam \leftarrow \RS(\bs_h, \gdparam)$.
        \STATE Compute reward $r = \log p_g(\bs_t ; \gdparam)$ and augment states $\hat \bs_t \leftarrow [\bs_t; \gdparam]$, $\hat \bs_{t+1} \leftarrow [\bs_{t+1}; \gdparam]$.
        \STATE Update $Q_\pq$ and $\pi_\ppi$ using $\gA$ and $(\hat \bs_t; \ba_t, \hat \bs_{t+1}, r)$.
    \ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

We call the method \textit{\METHOD} when learning a distribution from examples and \textit{\CMETHOD} when learning a conditional distribution.
We summarize both in \Cref{algo:disco}.

==> draft/6_experiments_short.tex <==
\section{Experiments}\label{sec:experiments}
Our experiments study the following questions:
\textbf{(1)} How does \METHOD with a learned distribution compare to prior work that also uses successful states for computing rewards?
\textbf{(2)} Can we apply \CMETHOD to solve long-horizon tasks that are decomposed into shorter sub-tasks?
\textbf{(3)} How do \METHODADJ policies perform when conditioned on goal distributions that were never used for data-collection?
The first two questions evaluate the variants of \METHOD presented in \Cref{sec:goal-distribution-inference}, and the third question studies how well the method can generalize to test time task specifications.
We also include ablations that study the importance of the relabeling strategy presented in \autoref{sec:learning-disco-policies}.

We study these questions in three simulated manipulation environments of varying complexity, shown in \autoref{fig:env-pictures}.
% For evaluation, we use a
We first consider a simple two-dimensional ``Flat World'' environment in which an agent can pick up and place objects at various locations.
The second environment contains a Sawyer robot, a rectangular tray, and four blocks, which the robot must learn to manipulate.
The agent controls the velocity of the end effector and gripper, and the arm is restricted to move in a 2D plane perpendicular to the table's surface.
Lastly, we use an IKEA furniture assembly environment from \citet{lee2019ikea}.
An agent controls the velocity of a cursor that can lift and place $3$ shelves onto a pole.
Shelves are connected automatically when they are within a certain distance of the cursor or pole.
The states comprise the Cartesian position of all relevant objects and, for the Sawyer task, the gripper state.
For the Sawyer environment, we also consider an image-based version which uses a 48x48 RGB image for the state.
% To accelerate learning on this image environment, we following past work on image-based RL~\citep{nair2018rig} and encode images $s$ with the mean of the VAE encoder $q_\encparam(\bz; \bs)$ for the RL algorithm and pretrain the VAE on 5000 randomly collected images.
All plots show mean and standard deviation across 5 seeds, as well as optimal performance (if non-zero) with a dashed line.

% \begin{figure}[t]
\begin{wrapfigure}{r}{0.6\textwidth}
    \vspace{-1.25cm}
    \centering
    \includegraphics[width=0.32\linewidth]{figures/screenshots/pointmass_env.pdf}
    \hfill
    \includegraphics[width=0.32\linewidth]{figures/screenshots/pybullet_task_fixed.pdf}
    \hfill
    \includegraphics[width=0.32\linewidth]{figures/screenshots/ikea_task_fixed.pdf}
    \hfill
    \caption{Illustrations of the experimental domains, in which a policy must
    (left) use the blue cursor to move objects to different locations,
    (center) control a Sawyer arm to move cubes into and out of a tray,
    and
    (right) attach shelves to a pole using a cursor.
    }
    \label{fig:env-pictures}
    \vspace{-0.25cm}
\end{wrapfigure}
% \end{figure}

\subsection{Learning from Examples}
Our first set of experiments evaluates how well \METHOD performs when learning distribution parameters from a fixed set of examples, as described in \Cref{sec:infer-from-examples}.
% To study the generality of \METHOD across different distribution parameterizations, 
We test all three parameterizations from \Cref{sec:goal-distribution-parameterization} on different environments:
First, we evaluate \METHOD with a Gaussian model learned via \Cref{eq:state-gd-inference} on the Sawyer environment, in which the policy must move the red object into the bowl and ignore three ``distractor'' objects.
Second, we evaluate \METHOD with a GMM model learned via \Cref{eq:state-gd-inference} on the Flat World environment, where the agent must move a specific object to any one of four locations.
Lastly, we evaluate \METHOD with a latent variable model learned via \Cref{eq:latent-space-gd-inference} on an image-based version of the Sawyer environment, where the policy must move the hand to a fixed location and ignore visual distractions.
This last experiment is done completely from images, where manually specifying the parameters of a Gaussian in image-space would be impractical.
The experiments used between $K=30$ to $50$ examples for learning the goal distribution parameters.
We report the normalized final distance, where we normalize by the final distance achieved by a random policy.
% In other words, a normalized distance of $1$ is no better than a random policy.

We compare to past work that uses example states to learn a reward function.
Specifically, we compare to variational inverse control with events (\textbf{VICE})~\citep{fu2018variational}, which trains a success classifier to predict the user-provided example states as positive and replay buffer states as negative, and then uses the log-likelihood of the classifier as a reward.
We also include an oracle labeled \textbf{SAC (oracle reward)} which uses the ground truth reward.
Since VICE requires training a separate classifier for each task, these experiments only test the methods on a single task.
Note that a single \METHOD policy can solve multiple tasks by conditioning on different distribution parameters, as we will study in the next section.

We see in \autoref{fig:single-task-results} that \METHOD often matches the performance of using an oracle reward and consistently outperforms VICE.
VICE often failed to learn, possibly because the method was developed using hundreds to thousands of examples, where as we only provided $30$ to $50$ examples.

\begin{wrapfigure}{r}{0.55\textwidth}
% \begin{figure}
    \vspace{-0.5cm}
    \centering
    \includegraphics[width=0.32\linewidth]{figures/plots/single-task/bullet_rel.pdf}
    \hfill
    \includegraphics[width=0.32\linewidth]{figures/plots/single-task/pg_gmm.pdf}
    \hfill
    \vspace{0.1cm}
    \includegraphics[width=0.32\linewidth]{figures/plots/single-task/visual-reacher.pdf}
    \includegraphics[width=0.70\linewidth]{figures/plots/single-task/legend.pdf}
    \hfill
    \caption{
    (Lower is better.)
    Learning curve showing normalized distance versus environment steps of various method.
    % Learning curve when inferring rewards from a set of example observations when 
    \METHOD uses a (left) Gaussian model, (middle) Gaussian mixture model, or (right) latent-variant model on their respective tasks. \METHOD with a learned goal distribution consistently outperforms VICE and obtains a final performance similar to using oracle rewards.
    }
    % \vspace{-0.075cm}
    % \vspace{-10pt}
    \label{fig:single-task-results}
% \end{figure}
\end{wrapfigure}

\subsection{Conditional Distributions for Sub-Task Decomposition}
The next experiments study how \CMETHOD can automatically decompose a complex task into easier sub-tasks.
We design tasks that require reaching a desired final state $\bs_f$, but that can be decomposed into smaller sub-tasks.
The first task requires controlling the Sawyer robot to move $4$ blocks with randomly initialized positions into a tray at a fixed location.
We design analogous tasks in the IKEA environment (with $3$ shelves and a pole) and Flat World environment (with $4$ objects).
All of these tasks can be split into sub-task that involving moving a single object at a time.

For each object $i=1, \dots, M$, we collect an example set $\dtask^i$.
As described in \Cref{sec:infer-conditional}, each set $\dtask^i$ contains $K=30$ to $50$ pairs of state $(\bs, \bs_f)$, in which object $i$ is in the same location as in the final desired state $\bs_f$, as shown in \Cref{fig:conditional-distribution-visualization}.
We fit a joint Gaussian to these pairs using \Cref{eq:learn-joint-distrib}.
During exploration and evaluation, we sample an initial state $\bs_0$ and final goal state $\bs_f$ uniformly from the set of possible states, and condition the policy on $\gdparam$ given by \Cref{eq:conditional-params}.
Because the tasks are randomly sampled,
% the specific task and goal distribution at evaluation time will have not seen during training time, and so
this setting also tested the ability for \CMETHOD to generalize to new goal distributions.

We evaluate how well \METHOD can solve long-horizon tasks by conditioning the policy on each \mbox{$p_g^i(\bs \mid \bs_f)$} sequentially for $H/M$ time steps.
We report the cumulative number of tasks that were solved, where each task is considered solved when the respective object is within a minimum distance of its target location specified by $\bs_f$.
For the IKEA environment, we also consider moving the pole to the correct location as a task.
We compare to VICE which trains separate classifiers and policies for each sub-task using the examples and also sequentially runs each policies for $H/M$ time steps.

One can train a goal-conditioned policy to reach this final state $\bs_f$ directly, and so we compare to hindsight experience replay (\textbf{HER})~\citep{andrychowicz2017her}, which attempts to directly reach the final state for $H$ time steps and learns using an oracle dense reward.
% Since HER does not decompose the task into subtasks, we expect that the learning will be significantly slowly since it does not exploit access to the tuples that give examples of a subtask being completed.
We see in \autoref{fig:long-horizon-results} that \CMETHOD significantly outperforms VICE and HER and that \CMETHOD successfully generalizes to new goal distributions.

\begin{wrapfigure}{r}{0.55\textwidth}
% \begin{figure}[t]
\vspace{-0.8cm}
\centering
    \includegraphics[width=0.32\linewidth]{figures/plots/multi_task/bullet_abs_oib.pdf}
    \hfill
    \includegraphics[width=0.32\linewidth]{figures/plots/multi_task/ikea.pdf}
    \hfill
    \vspace{0.1cm}
    \includegraphics[width=0.32\linewidth]{figures/plots/multi_task/pg.pdf}
    \includegraphics[width=\linewidth]{figures/plots/multi_task/legend.pdf}
        
    \caption{(Higher is better.) Learning curves showing the number of cumulative tasks completed versus environment steps for the Sawyer (left), IKEA (middle), and Flat World (right) tasks. We see that \METHOD significantly outperforms HER and VICE, and that relabeling the mean and covariance is important.
    }
    \label{fig:long-horizon-results}
    \vspace{-1.25cm}
% \end{figure}
\end{wrapfigure}

\paragraph{Ablations}
Lastly, we include ablations that test the importance of relabeling the mean and covariance parameters during training. % using \autoref{eq:conditional-relabelling}.
We see in \autoref{fig:long-horizon-results} that relabeling both parameters, and particularly the mean, accelerates learning.


==> draft/90_notes.tex <==
\section{Method Notes (not for paper)}

\subsection{Generalized Goal Specification and Inference}

The aim of the agent is to maximize the likelihood of the current state $p_g(s; \theta)$ according to a goal distribution $p_g$ parametrized by $\theta$.

How to infer $\theta$ is a separate problem; it may be inferred by maximum likelihood from a dataset $\mathcal{D}$ - for instance, goal images or expert trajectories. It may also be conditioned on the state observation $s$ - for instance, if a goal state is provided or some other input such as language specification. So in general, $\theta = f(\mathcal{D}, s)$. The advantage of breaking up RL into this two phase inference procedure (which may be interleaved, eg. in IRL) is that it disentangles reward learning with dynamics learning in a way that enables us to use sample-efficient GCRL algorithms. Going forward, let's split the state observation into $s$, the Markovian state of the MDP, and $c$, a context independent of $s$ which affects the reward function.

\subsection{Goal Inference with IRL}
In this section, we have a dataset of trajectories $\mathcal{D} = \{\tau_1, \tau_2, \dots, \tau_N\}$ and want to recover a (goal-conditioned) reward function and policy. Everything is in terms of $\tau$ below, but since we only care about $r(s)$ I think it can all be in terms of single-step transitions just as easily. We want to assume the goal distribution are simple, ie. $p_g$ is Gaussian with few parameters.

\subsubsection{Single-Task IRL}
In the framework of max-ent IRL, $p(\tau; \theta) = \exp(r(\tau))/Z(\theta)$, where $Z(\theta) = \int \exp(r(\tau)) d\tau$. Assuming the reward does not depend on a context, $r(\tau) = \log p_g(\tau; \theta)$ and we can write $\log p(\tau; \theta) = -\log Z(\theta) + \log p_g(\tau; \theta)$.
% \sum_{t=0}^T \log p_g(s_t; \theta)$.

We then want to learn the parameters $\theta$ that maximize the likelihood of the dataset:
$\max_\theta \E_{\tau \sim \mathcal{D}}[p(\tau; \theta)] = \E[-\log Z(\theta) + \log p_g(\tau; \theta)]$

$Z(\theta)$ can be estimated by sampling trajectories that optimize $r_\theta$, inducing the usual IRL alternating optimization. In one phase, we do RL; in the other phase, we update $\theta$ according to the above. In other words we iterate between step 2 and 4 below:
\begin{align}
    & \max_\theta \E_{\tau \sim \mathcal{D}}[p(\tau; \theta)] = -\log Z(\theta) + \E_{\tau \sim \mathcal{D}}[\log p_g(\tau; \theta)] \\
    & \; \; \log Z(\theta) = \log \E_{\tau \sim \pi}[\frac{\log p_g(\tau)}{\pi(\tau)}] \\
    & \max_\pi \E_{\tau \sim \pi}[\log p_g(\tau)]
\end{align}

The parameters of $\theta$ should be simple. So, we can actually do GCRL to capture a wide distribution of $\theta$, which means the inner-RL loop can be cheap (at the limit you train RL once at the start and only sample from the learned policy afterwards). \textbf{So even in the single task setting, you could benefit from the policy being conditioned on $\theta$,} basically because $\theta$ is being changed in the IRL optimization.

Showing we can do this with goal distributions, and that its better than using a generic function $r_\theta(s)$ could be a good way to show how goal distributions are useful.

What base IRL algorithm to use? - maybe AIRL. In this case we would be estimating eqn 2 by learning a discriminator between trajectories from $\pi$ and $\mathcal{D}$.

\subsubsection{IRL + Representation Learning}

What if the reward cannot be expressed as a simple distribution (eg. Gaussian) in the state space? Then we can learn an intermediate representation for goals. The procedure is the same as above, but introducing a latent variable $z \sim q_\phi(z|s)$. Goals are now in latent space; ie. now we learn $p_g(z_t; \theta)$. This is the new optimization:
\begin{align}
    & \max_{\theta, \phi} \E_{\tau \sim \mathcal{D}}[p(\tau; \theta)] = -\log Z(\theta) + \E_{\tau \sim \mathcal{D}}[\log p_g(\tau; \theta)] + \KL(q_\phi(z|s)||p(z)) \\
    & \max_\pi \E_{\tau \sim \pi}[\log p_g(\tau)]
\end{align}

This formulation would be fully general, in the sense that the latent variable could in theory learn any arbitrary reward $r(s)$ as a single element. But if $r(s)$ is more easy to express as a norm, it should instead learn that.

Are there any degenerate solutions? (Are they fixed by having $z$ reconstruct the state?)

\subsubsection{IRL + multi-task}

What if instead you have a contextual/multitask/goal-conditioned task where reward is $r(s, c)$. Now instead of inferring a single distribution $\theta$, you need to train $q_\psi(\theta|c)$. Prior work like HER assumes this is the identity, but it could be much more - eg. if $c$ is some language instructions. This is the new optimization:
\begin{align}
    & \max_{\theta, \phi, \psi} \E_{\tau \sim \mathcal{D}}[p(\tau; \theta)] = \E_{\theta \sim q_\psi(\theta|c)}[-\log Z(\theta) + \E_{\tau \sim \mathcal{D}}[\log p_g(\tau; \theta)]] + \KL(q_\phi(z|s)||p(z)) \\
    & \max_\pi \E_{\tau \sim \pi}[\log p_g(\tau)]
\end{align}

One issue is that if $\psi$ is complex, eg. a neural network, maybe it would be quite sample-inefficient to learn even something simple like the identity.

Again, need to consider if there are any degenerate solutions.

\subsection{Setting}

Consider a multi-step task with $N$ stages and a step reward $r(s, g) \in \{0, 1, \dots, N\}$. We start with an initial dataset $\gD = \{\gS_0, \gS_1, \dots, \gS_N,\}$ where $\gS_i$ is composed of state-goal tuples that satisfy $r(s, g) = i$. We will start with true state, but eventually want states and goals to be images.

This dataset may naturally be collected by labeling (demonstration) trajectories with rewards and considering the last observation as the goal. But it may be that collecting just the images is less cumbersome.

The aim is to recover a policy that maximizes $\E[\sum_t r(s, g)]$, although we never observe the true reward during training time after the initial dataset. (We can also consider settings where we do mostly self-supervised learning but intermittently get labeled rewards for the agent's trajectories.)

\subsection{Practicing Skills with Goal Distributions}

In order to independently practice sub-skills of the entire task, we will infer a set of waypoint distributions $\{W_{ij}\}, W_{ij} \sim p_{\theta_{ij}} = \mathcal{N}(\mu_{ij}, \Sigma_{ij})$ corresponding to the achieving the specific sub-skill of stage $j$ while going from stage $i$ to the goal $g$ of the task.

For a particular waypoint $W$, the reward will be $r = \log p_W(s) = -||\Sigma^{-1/2}(s - \mu)||^2$ omitting irrelevant terms (this is the negative squared Mahalanobis distance). The policy and Q function will be conditioned on these parameters in order to generalize across them: $\pi(a|s, \theta)$ and $Q(s, a, \theta)$.
At rollout time we can randomly sample $\theta_{ij}$ in order to collect coherent, meaningful samples. 
At test time, we could relabel with the same mixture distribution, or potentially consider a wider goal distribution.

We might fit these goal distributions directly to data, for instance by fitting the mean and covariance of examples from a particular stage. But for the tasks we are considering, the sub-goal distribution of interest is innately linked to the current state and final goal. To fit these waypoints, instead we should fit a density model to $p(s, w_{ij}, g)$ from the demonstrations, and then at rollout time infer $p(w_{ij}|s, g)$.

There are likely many choices for inferring $p(w_{ij}|s, g)$.

\subsection{Off-Policy RL}

The idea is that we treat $\{\theta_j\}$ as another thing we can sample for exploration and relabel off-policy while training, just like goals. We learn a policy $\pi(s, g, \theta)$ and action-value function $Q(s, g, \theta)$. When doing exploration, sampling various $\theta$ should allow us to do directed exploration for each subtask independently. But all data can be used to learn any of the subtasks due to off-policy relabeling. At test time, we evaluate $\theta_j$ corresponding to $H_{N-1}$.

How to trade-off between subtasks ($L_i$) and cumulative tasks ($H_i$) could be an interesting question. For now, maybe we can just treat them uniformly. 


\subsection{Notes on representation Learning version \VP{not for paper}}
Let $\set$ denote a set of observations, $\set = \{x_s, \dots, x_{|\set|}\}$.
Assume we have $S$ such sets $\{\set_s\}_{s=1}^S$.
We would like to learn an encoding of the observations $\enc: \mathcal{X} \rightarrow \mathcal{Z}$ such that we can model each set as a Gaussian distribution in a latent space.
In other words, we would like
\begin{align}
    % \log p(x_i^{(s)} \mid 0
    \{\enc(x_i^{(s)})\}_{i=1}^{|\set_s|}
\end{align}
to look like a factorized Gaussian.

\paragraph{Approach 1: VAE + regularization.}
Train a normal VAE, but add a regularization penalty that that encourages points in set to ``be similar.'' This similarity could be encouraged by
\begin{itemize}
\item penalizing the pair-wise KL divergence between observations from the same set
\item rewarding the pair-wise KL divergence between observations from different sets
\end{itemize}

\paragraph{Approach 2: Set-based VAE.}
Train an encoder that's conditioned on a set, and then train the decoder to reconstruct multiple images simultaneously.

So we could have $q(z \mid \set)$ and use it to maximizing $\E_{z \sim q} \left[ \log p_\theta(\set \mid z) \right]$.
To evaluate the likelihood, we could sample a single $z$ and then evaluate
\begin{align*}
	\sum_{x_i \in \set} \log p_\theta(x_i \mid z), z \sim q(z \mid \set)
\end{align*}
or we could sample one $z$ per example and evaluate
\begin{align*}
	\sum_{x_i \in \set} \log p_\theta(x_i \mid z_i), z_i \overset{iid}{\sim} q(z \mid \set)
\end{align*}
yet another approach would be to ``match'' each $z_i$ sample with the corresponding $x_i$ that maximizes its likelihood
\begin{align*}
	\sum_{x_i \in \set}\max_{z \in {Z}} \log p_\theta(x_i \mid z)\\
    Z = \{z_i\}, z_i \overset{iid}{\sim} q(z \mid \set)
\end{align*}

\paragraph{Approach 3: Auto-encoder + distribution penalty.}
 Train an autoencoder to maximize reconstruction and minimize the total correlation:
\begin{align*}
    \max_\theta \sum_i \left( \log p(x_i \mid z_i) \right) - C(Z[1], Z[2], \dots, Z[3]), z_i = \enc_\theta(x_i)
\end{align*}
This total correlation might not be too hard to approximate. We could, for example, fit a Gaussian to the joint distribution of latent encodings, and then fit marginal distributions to each latent dimension. Then (I think) we could take the KL between the two.

\paragraph{Approach 4: EM-style}
In this approach, we basically treat this as an EM problem, where the mean and variance of the latent distribution (the generative model) are unknown, and we need to jointly learn to map each $x_i$ to $z_i$ (the ``latent variable'').
We alternative between computing parameters that maximize the likelihood of the encodings:
\begin{align*}
    \mu_z &= \text{mean}(z_1, \dots, z_N)\\
    \Sigma_\text{joint} &= \text{Covariance}(z_1, \dots, z_N)
\end{align*}
and training some decoder. This might end up being the same as Approach 2, but without the prior KL penalty.


==> draft/95_method_conditional_distribution.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    % \includegraphics[width=\linewidth]{figures/stub/representation_learning_procedure.png}
    \includegraphics[width=\linewidth]{figures/stub/conditional_distribution.png}
    % \caption{(Left) Given the final task of ___ that requires reaching a goal state $\bs_f$, a robot must complete the subtask of ___, for which there exist multiple states $\bs$.  (Right) We use pairs of states $\bs, \bs_f$ to learn a conditional distribution, $\pg$}
    \caption{(Left) A robot must arrange objects into a specific configuration $\bs_f$, that changes from episode to episode.
    This task consists of multiple sub-tasks, such as first moving the red object to the correct location.
    Given a final state $\bs_f$, there exists a distribution of intermediate states $\bs_r$ in which this first sub-task is completed.
    (Right) We use pairs of states $\bs_r, \bs_f$ to learn a conditional distribution that defines the first sub-task given the final task, \mbox{$p(\bs_r \mid \bs_f)$}.}
    \label{fig:conditional-distribution-visualization}
\end{wrapfigure}

While inferring goal distributions from a single set can be used to describe many problems, in robotics we are particularly interested in multi-step tasks that can be specified by a final state $\bs_F$. For instance, consider the task of arranging a dinner table given a final desired goal state $\bs_f$ that specifies the location of every piece of silverware. In this case, we want to separate the task into steps, and be able to describe each step $i$, such as moving a plate to its target location, by a separate distribution parametrized by $\gdparam_i$: $p(\bs|\bs_F; \omega_i)$. Note that the acceptable intermediate states to reach $\bs_F$ depend on $\bs_F$; thus instead of the parameters $w$ being independent as in the previous section, $\gdparam_i = h(\bs_F)$ will in this section be a function of $\bs_F$. Once inferred, a DisCo policy $\pi(a|s, s_F, \gdparam)$ is trained to solve the goal-reaching problem.

Concretely, we assume that for a particular step $i$, a user provides pairs of observations $\{(\bs^{(k)}, \bs_f^{(k)})\}_{k=1}^K$, in which $\bs^{(k)}$ correspond to a state where a sub-task is accomplished when trying to reach the final state $\bs_f$.
We first fit a joint Gaussian distribution, denoted by \mbox{$p(\bs, \bs_f)$}, to these pairs of states. Then, given a target state $\bs_f$ to reach at exploration or test time, we compute the conditional distribution \mbox{$p_{\bS \mid \bS_f}(\bs \mid \bs_f; \gdparam_i)$}.
Since the joint distribution $p_{\bS, \bS_f}$ is Gaussian, the conditional distribution $p_{\bS | \bS_f}$ is also Gaussian with parameters $\omega = h(\bS_f)$, where $h$ is the standard conditional Gaussian formula.\footnote{
If $\bS, \bS_f \sim \gN\left(
\begin{bmatrix}\mu_1 \\ \mu_2 \end{bmatrix}
,
\begin{bmatrix}
\Sigma_{11} & \Sigma_{12} \\
\Sigma_{21} & \Sigma_{22} \\
\end{bmatrix}
\right)
$
% then
% $X_1 \mid X_2 \sim \gN\left(
% \mu_1 + \Sigma_{12} \Sigma_{22}^{-1}(X_2 - \mu_2),
% \Sigma_{11} - \Sigma_{12}\Sigma_{22}^{-1}\Sigma_{21}
% \right)$
,
then
$\bS \mid \bS_f \sim \gN(\omega)$ where
$\omega = h(\bS_f) = (
\mu_1 + \Sigma_{12} \Sigma_{22}^{-1}(\bS_f - \mu_2),
\Sigma_{11} - \Sigma_{12}\Sigma_{22}^{-1}\Sigma_{21}
)
$
% $\hat \mu = \mu_1 + \Sigma_{12} \Sigma_{22}^{-1}(X_2 - \mu_2)$
% and
% $\hat \Sigma = \Sigma_{11} - \Sigma_{12}\Sigma_{22}^{-1}\Sigma_{21}$
.
}

%~\citep{page1984multivariate}.

% can be computed in closed form, and is given by Gaussian distribution with parameters $\omega = g(\bS_f)$, where $g$ is the standard funciton.
% Yet another approach would be to learn a conditional distribution $p_f(\bs \mid \cparam)$ where $\cparam$ is some additional parameter to dynamically select the goal distribution.
% In our experiments, we find that both of these approaches work well.
% This can allow a policy to generalize to new contexts $c$.
%%GB.7.21: This section is bit rough around the edges. Which method do we use, lets not say two methods can be used, it makes it sound like we are not sure what we are doing. This does not 
% \paragraph{Manual-specification}
% \paragraph{MLE}

This conditional distribution also provides a simple way to relabel goal distributions.
Given a state $\bs_t$ that was reached in a trajectory, we relabel the goal distribution by using the parameters $\omega=h(\bs_t)$.

----

Any way of generating distributions is a valid way of generating a task for a \METHODADJ policy.
In this section, we consider a particularly useful way of generating a distribution: conditional distributions.
With conditional distributions, the parameter $\gdparam$ is generated by first computing a conditional distribution $p(\bs | X)$, for some random variable $X$ and then extracting the corresponding parameters $\omega$ out of this distribution.
Conditional distributions are useful since they allow a user to dynamically generate different distributions, based on the conditioning random variable $X$.

One promising application of this conditional distribution formulation is to facilitate learning goal-directed behavior, in particular when tasks can be decomposed into multiple stages.
For example, as we visualize in \autoref{fig:conditional-distribution-visualization} a robot that must arrange a dinner table may have a final desired goal state $\bs_f$ that specifies the location of every piece of silverware, but this task can be decomposed into several sub-tasks, such as placing one plate in a desired location, each of which can be expressed as a \METHOD problem.
This decomposition can make learning significantly easier, compared to training a single policy to directly reach $\bs_f$.
% Decomposing a long-horizon problem into several easier components can significantly easier to train such a policy.
% Another use case for \METHOD is when there exists a single task, such as 
% While this can be
In this situation, we need a way to generate a goal distribution for each sub-task, conditioned on the random variable, $\bs_f$, the final desired state.
% While \METHOD is a more general framework than goal-conditioned RL, it can also be used 
% In other words, we would like to obtain \emph{conditional} probability distributions.
% Fortunately, conditional probability distributions capture this precise use case: given a goal state $\bs_f$, what is the distribution

While \METHOD is a more general framework than goal-conditioned RL, it can also be used to facilitate learning goal-directed behavior, in particular when tasks can be decomposed into multiple stages.
For example, as we visualize in \autoref{fig:conditional-distribution-visualization} a robot that must arrange a dinner table may have a final desired goal state $\bs_f$, that specifies the location of every piece of silverware, but this task can be decomposed into several sub-tasks, such as placing one plate in a desired location, each of which can be expressed as a \METHOD problem.
This decomposition can make learning significantly easier, compared to training a single policy to directly reach $\bs_f$.
In this situation, we need a way to generate a goal distribution for each sub-task, conditioned on a final state $\bs_f$.
% In other words, we would like to obtain \emph{conditional} probability distributions.
% Formally, we want to infer the parameters of the conditional distribution $p(s|s_F)$ rather than $p(s)$. 

Formally, we want to find a map $h: \gS \mapsto \gdspace$ that maps a final state $\bs_f$ to a goal distribution parameter $\gdparam$ that represents a sub-task for reaching $\bs_f$.
This map allows us to dynamically generate distributions over the state space conditioning on $\bs_f$, by mapping a state $\bs_f$ into a distribution parameter $\omega = h(\bs_f)$.
One way we can the function $h$ is to learn a conditional distribution $p_{\bS \mid \bS_f}$, which maps an observation of the random variable $\bs_f$ into a probability distribution over the state space.

% Formally, we want to create a conditional distribution $p(\bs \mid \bs_f)$, which
% This conditional distribution allows us to dynamically generate distributions over the state space conditioning on $\bs_f$, by mapping a state $\bs_f$ into a distribution paramter $\omega = h(\bs_f)$.
% We need $h$
To obtain this conditional distribution, we assume that a user provides pairs of observations $\{(\bs^{(k)}, \bs_f^{(k)})\}_{k=1}^K$, in which $\bs^{(k)}$ correspond to a state where a sub-task is accomplished when trying to reach the final state $\bs_f$.
% We fit a joint Gaussian distribution, denoted by \mbox{$p_{\bS, \bS_F}(\bs, \bs_f)$}, to these pairs of states.
We fit a joint Gaussian distribution of the form
\begin{align*}
p_{\bS, \bS_f} = 
\gN
\left(
\begin{bmatrix}\mu_\bs \\ \mu_{\bs_f} \end{bmatrix}
,
\begin{bmatrix}
\Sigma_{\bs \bs} & \Sigma_{\bs \bs_f} \\
\Sigma_{\bs_f \bs} & \Sigma_{\bs_f \bs_f} \\
\end{bmatrix}
\right),
\mu_{(\cdot)} \in \R^{\text{dim}(\gS)},
% \Sigma_{\bs\bs}
% \Sigma_{\bs_f \bs}
% \Sigma_{\bs \bs_f}
% \Sigma_{\bs_f \bs_f}
\Sigma_{(\cdot)}
\in \R^{\text{dim}(\gS) \times \text{dim}(\gS)}
% \mu_s \in \R^{|\gS|}
\end{align*}
to these pairs of states using maximum likelihood estimation.
% and then compute the conditional distribution \mbox{$p_{\bS \mid \bS_f}(\bs \mid \bs_f)$}.
Since the joint distribution $p_{\bS, \bS_f}$ is Gaussian, the conditional distribution $p_{\bS | \bS_f}$ is also Gaussian with parameters $(\mu, \Sigma) = h(\bs_f)$, where $h$ is the standard conditional Gaussian formula:
\begin{align}\label{eq:conditional-relabelling}
h(\bs_f) = \left( 
\underbrace{
\mu_\bs + \Sigma_{\bs \bs_f} \Sigma_{\bs_f \bs_f}^{-1}(\bs_f - \mu_{\bs_f})
}_{\mu}
,
\underbrace{
\Sigma_{\bs \bs} - \Sigma_{\bs \bs_f}\Sigma_{\bs_f \bs_f}^{-1}\Sigma_{\bs_f \bs}
}_{\Sigma}
\right).
\end{align}
% If $\bS, \bS_f \sim \gN\left(
% \begin{bmatrix}\mu_1 \\ \mu_2 \end{bmatrix}
% ,
% \begin{bmatrix}
% \Sigma_{11} & \Sigma_{12} \\
% \Sigma_{21} & \Sigma_{22} \\
% \end{bmatrix}
% \right)
% $
% then
% $X_1 \mid X_2 \sim \gN\left(
% \mu_1 + \Sigma_{12} \Sigma_{22}^{-1}(X_2 - \mu_2),
% \Sigma_{11} - \Sigma_{12}\Sigma_{22}^{-1}\Sigma_{21}
% \right)$
% ,
% then
% $\bS \mid \bS_f \sim \gN(\omega)$ where
% $\omega = h(\bS_f) = (
% \mu_1 + \Sigma_{12} \Sigma_{22}^{-1}(\bS_f - \mu_2),
% \Sigma_{11} - \Sigma_{12}\Sigma_{22}^{-1}\Sigma_{21}
% )
% $
% $\hat \mu = \mu_1 + \Sigma_{12} \Sigma_{22}^{-1}(X_2 - \mu_2)$
% and
% $\hat \Sigma = \Sigma_{11} - \Sigma_{12}\Sigma_{22}^{-1}\Sigma_{21}$
In summary, given a final desired state $\bs_f$, we generate a distribution by computing \mbox{$\gdparam = h(\bs_f)$} according to \autoref{eq:conditional-relabelling}.
This conditional distribution also provides a simple way to relabel goal distributions given a reached state $\bs_r$:
we relabel the goal distribution by using the parameters \mbox{$\omega' = h(\bs_r)$}.
% Given a state that was reached $\bs_f$, we relabel the goal distribution by using the parameters \mbox{$\omega' = h(\bs_f)$}.
%~\citep{page1984multivariate}.
% can be computed in closed form, and is given by Gaussian distribution with parameters $\omega = g(\bS_f)$, where $g$ is the standard funciton.
% Yet another approach would be to learn a conditional distribution $p_f(\bs \mid \cparam)$ where $\cparam$ is some additional parameter to dynamically select the goal distribution.
% In our experiments, we find that both of these approaches work well.
% This can allow a policy to generalize to new contexts $c$.
%%GB.7.21: This section is bit rough around the edges. Which method do we use, lets not say two methods can be used, it makes it sound like we are not sure what we are doing. This does not 
% \paragraph{Manual-specification}
% \paragraph{MLE}
% of \mbox{$p_{\bS \mid \bS_f}(\cdot \mid \bs_f)$}.

% In some domains and tasks, the corresponding reward function is not proportional to a Gaussian distributions.
% For example, consider environments where a states correspond to images, and a user provides a set of example images in which a task is completed.%, though the following procedure is also applicable to any environment including non-image ones.
% Fitting a Gaussian distribution to images is unlikely to produce meaningful rewards.
% In order to obtain meaningful rewards, we would like to embed images, or more generally states, into a learned latent representation where Gaussian distributions are more meaningful.


==> draft/96_old_experiments.tex <==
%%SL.7.17: It would be a good idea to sketch out the experiment results figures as soon as possible, so that we understand what figures we have to make
% \begin{figure}
%     \begin{subfigure}[b]{0.4\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/screenshots/pg.png}
%         \caption{\PYGAME}
%         \label{fig:2d-env-picture}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.4\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/screenshots/bullet.png}
%         \caption{\PYBULLET}
%         \label{fig:sawyer-picture}
%     \end{subfigure}
%     \caption{Caption}
% \end{figure}
% We will perform the following experiments
% \begin{enumerate}
%     \item (the ``$p(\omega)$'' version) First we want to show that the method works and ideal outperforms GCRL and VICE on goals that are relative positions. We should perform two versions of this experiment: one with a sliding box and one object and another with one object, 3 distractors, and fixed box. We can give GCRL an "oracle" goal that comes from sampling the GDCRL distribution. VICE will be trained using the expert set used to infer the distribution. \todo{This means that All experiments should used inferred distributions for a fair comparison to VICE and GCRL}
%     \item (the ``$p(\omega \mid c )$'' version) Next we want to show where goal distribution come from and how they can be used and can result in some generalization. In this case we want to show that if we condition $p(\omega|c)$ we can learn a more interesting distribution and possibly generalize over $c$s not seen during training. This experiment will also show that the method works better than GCRL and VICE (partly due to the many distractors).
%     \item (ablations) This is with the same motivation as the last experiment but we can also check how our relabeling strategies affect performance. This is additional context on how the distributions are used and allow us to learn more principled exploration.
%     \item (representation learning) GDCRL can in principal represent any reward function. For this we combine GDCRL with a VAE (or some kind on non-linear transformation of the state space) to show that the method works and still infers proper task distributions. It would be great if we can have these results for images but we can start with a true state VAE (this will help validate that the distribution inferring method still works).
%     % \item We show that this method has additional application advantages. In this case we show that the method can plan better using GDCRL and GCRL (I don't see an easy way to compare this to VICE, without training a bunch of policies...). These methods will be compared over their ability to accomplish a prescribed plan (given with 4 sub goals, we should sample many different plans so we have a more reasonable approximation of performance and are not biased to any particular plan or ordering). 
% \end{enumerate}

\paragraph{Generalization to initial states.}
To evaluate our method's ability to generalize to new states, we consider a task in which the location of the bowl varies at the beginning of each episode, and the agent must always move the first object into the bowl without regard for the location of the other three objects.
%%SL.7.23: I would recommend writing the task description more carefully. Right now the task seems really simple, and is not well explained. It's important to explain clearly why the task is challenging and interesting, and ideally illustrate it with some pictures. Perhaps remarking that the goal-conditioned policy struggles with it would help to make the point.
At the beginning of each episode, we sample a new initial state, collect data with the policy for $H$ time steps, and measure the final distance between the first object to the bowl's center location.
%%SL.7.23: Above sentence is a bit unclear, sounds like we measure the distance on the initial state.
% The agent must learn to ignore three of the objects and must also learn to move the first obj
% Note that this task cannot be expressed as a single goal state, since three of the objects must be ignored, and the task is only defined in terms of the relative positions between the first object and the bowl.
% Note that this task cannot be expressed as a single goal state, since three of the objects must be ignored, and the task is only defined in terms of the relative positions between the first object and the bowl.

%%SL.7.23: I would recommend having a paragraph at the beginning (before the initial states section) to explain what are the baselines and comparisons and introduce their acronyms, so that we can reference them in the material below.

First, we study how standard goal-conditioned reinforcement learning methods perform on this task.
This task cannot be expressed as a single goal states, since the location where the object must be placed depends on the location of the box, which is unknown until the beginning of the episode.
% While this task cannot be expressed as a single goal states,
%%SL.7.23: why?
Of course, for any given initial state, one can choose a nearby goal state that accomplishes the task.
%%SL.7.23: It's a bit unclear why you are suddenly talking about this, perhaps preface this by saying something like: First, we study how standard goal-conditioned reinforcement learning methods perform on this task.
However, this requires an oracle that can be queried at the beginning of every rollout.
While our method does not require such an oracle, we provide it to the GCRL baseline, which we label as \textbf{GCRL + Oracle}.
To obtain a goal distribution, we perform maximum likelihood estimation to estimate the goal distribution parameter
%%SL.7.23: maximum likelihood what?
$\gdparam^*$ using a set of $N=30$ observations, in which the first object is in the bowl.

The results are shown in \autoref{fig:state-generalization-results}, and we see that \METHOD significantly outperforms GCRL even with the oracle.
We found that GCRL failed because it primarily focused on moving the hand to the correct location, without first picking up the object.

%%SL.7.23: I think this discussion of the results is a bit terse. What was the distribution learned by our method? What does it look like? Do we have a picture of the execution? A picture of what the baseline does? Some kind of analysis to understand how the methods are performing? I think it's also likely that some reviewers will complain about reproducibility, such as missing details about how the GCRL baseline is set up, environment parameters, number of time steps, etc. (which could go in the appendix)

% In contrast the distribution learned by 

% \begin{itemize}
%     \item objective: evaluate method's ability to generalize to new states
%     \item env setup: PnP, random box position at initial state, box can move but this is suboptimal, 4 objects, put 1 object in the box, and always ignore other 3.
%     \item why it's hard: the optimal behavior depends on the initial state, and there's no single fixed goal position
%     \item exploration: (our method has no samples)
%     \item our method, training: future-style relabeling of the mean
%     \item baseline, exploration and evaluation: Goal-conditioned reinforcement learning (\textbf{GCRL}) is sampling from the example set
%     \item algorithmic setup: To obtain goal distributions, we use the MLE + thresholding procedure describe in \autoref{sec:goal-distribution-inference} once.
%     \item results: \autoref{fig:bullet-results}
%     \item conclusion: TODO
% \end{itemize}

\paragraph{Generalization to new goal distributions.}
To evaluate our method's ability to generalize to new distribution,
To evaluate how well a single \METHODADJ policy can generalize to new goal distributions at test time, we consider a task in which the location of the bowl is fixed, and the agent must move one of the four objects to target locations.
% In order to test generalization to new goal distributions, we need a way to generate goal distributions.
%%SL.7.23: ...that seems like a pretty obvious (and therefore unnecessary) statement
While we could manually specify a procedure for sampling goal distribution parameters $\gdparam = (\mu, \Sigma)$, we can automate this process and more directly compare to goal-conditioned RL by automatically constructing a goal distribution, conditioned on a given goal state $\bs_g$.
%%SL.7.23: Maybe for this part it's OK to just describe this procedurally, instead of saying "While we could..." (i.e., "For evaluation [or training?], we construct the tasks procedurally by [whatever]")
Given a goal state $\bs_g$, which specifies the location of all four objects, there is
%%SL.7.23: "there is" seems like the wrong clause here
a distribution of states $p_1(\bs \mid \bs_g)$ in which the first object is in the same location as in the goal state $\bs_g$.
Similarly, there is
%%SL.7.23: same comment
another distribution of states, $p_2(\bs | \bs_g)$, in which the second object is in the same location as in the goal state $\bs_g$.
As we vary $\bs_g$, these conditional distribution will vary, providing a simple way to generate a continuum of goal distributions.
%%SL.7.23: Can we revise the above paragraph for clarity, and include a figure that shows the tasks that are generated? A picture is likely worth a thousand words here.
% In other words, we obtain a spectrum of goal distributions by learning conditional distribution $\$

% While we could manually specify a procedure for sampling the goal distribution parameters $\mu, \Sigma$, we use the conditional formulation discussed in \autoref{sec:goal-distribution-inference}, where $\cparam$ corresponds to a goal state $\bs_g$.
For each object, we fit a normal distribution $p_i(\bs, \bs_g)$ to a dataset in which $\bs$ is a waypoint for reaching a goal $\bs_g$ and the $i$th object is already in the correct position.
%%SL.7.23: Again, a figure clarifying this would really help
We then obtain a conditional distribution by computing $p_i(\bs \mid \bs_g)$, which can be done in closed form.
At the beginning of each episode, we sample a new initial state, sample a goal state $\bs_g$,
%%SL.7.23: from where? maybe don't use the word sample if it is selected (as part of the evaluation) rather than sampled from a distribution learned by our method or something
condition a \METHODADJ policy on the parameters of the distribution $p_i(\bs \mid \bs_g)$, and measure the final distance between the $i$th object to its intended direction in $\bs_g$.
Different goal states give rise to different goal distributions $p_i(\bs \mid \bs_g)$, allowing us to test generalization to new goal distributions.
For comparison, we train GCRL to reach the goal state $\bs_g$ and similarly report its final final distance to the $i$th object.
%%SL.7.23: It's not entirely clear that this is a fair comparison
For the plots, we average $i$ over all four objects.

We see in \autoref{fig:distribution-generalization-results} that \METHOD significantly outperforms the goal-conditioned baseline and successfully generalizes to new goal distributions at test time.
We found that, similarly to the results in the previous section, the goal-conditioned policy focuses primarily on the location of the arm, failing to manipulate the objects properly.
%%SL.7.23: I don't know if there is anything we can do about it this late in the process, but a likely concern that reviewers will have at this point in the paper is that we somewhat low-balled the comparisons. In all the evaluations, the goal-conditioned policy fails utterly, which might make the reviewers suspect that we simply did not implement it correctly.
% \begin{itemize}
%     \item objective: evaluate method's ability to generalize to new distributions (new means)
%     \item env setup: PnP, fixed box position always, 4 objects, 4 different distributions
%     \item why it's hard: the optimal behavior depends on the initial state, and there's no single fixed goal position, must ignore many things
%     \item exploration: context $c$ is sampled, 50\% of the time we cycle through the policies (atomic sequential), 50\% we choose one randomly and stick with it (atomic)
%     \item training: future-style relabeling of the mean
%     \item for sampling the context $c$, training/exploration: 50\% of the time, all object are inside the box. 50\% of the time, all the objects are anywhere on the ground (which could be in the box)
%     \item our method evaluation: only run with one distribution and evaluate final distance for that object (currently, the plots always have $c$ = all objects in box, but ideally we'll also test other $c$s)
%     \item GCRL baseline, training/exploration: same sampling of $c$ as our method during training/exploration
%     \item GCRL baseline, evaluation metric: currently just takes one of the objects, but ideally we'll take the min distance across all the objects
%     \item algorithmic setup: To obtain goal distributions, we learn $p(w | c)$
%     \item results: \autoref{fig:bullet-results}
%     \item conclusion: TODO
% \end{itemize}

\begin{figure}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/plots/bullet_rel.pdf}
        \caption{Initial state generalization results.}
        \label{fig:state-generalization-results}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/plots/bullet_abs.pdf}
        \caption{Distribution generalization results.}
        \label{fig:distribution-generalization-results}
    \end{subfigure}
    \caption{\PYBULLET \TODO{fill}}
\end{figure}
%%SL.7.23: See writing guide regarding how to write a caption
% Comparisons:
% \begin{enumerate}
%     \item VICE: VICE is a method for solving one specific task. So in the $p(\omega \mid c)$
% \end{enumerate}

%%SL.7.23: Any way we could repeat this experiment in the Sawyer environment?
\paragraph{Ablations.}
We also perform ablative studies on a simplified \textit{\PYGAME} domain, where it is more computationally feasible
%%SL.7.23: This doesn't come across as very convincing -- why is it not feasible in the Sawyer environment?
to run extensive comparisons in which we can study the impact of different design decisions.
As shown in \autoref{fig:2d-env-picture}, this environment comprises (1) a blue circular cursor which can move around in a 2D arena and (2) four circular objects placed around the arena which must be moved arbitrary locations.
The agent can interface with the cursor by specifying 2D velocity, and also a continuous grasp action between $-1$ and $1$.
When the grasp action non-negative, the agent will ``grab'' the nearest object within a small radius of its current location.
This object will move with the cursor until the agent releases the object by emitting a negative grasp action.
The state contains the XY-position of the cursor and the objects.

At the beginning of each episode, the initial states is sampled uniformly from the set of possible states, and the agent must move one of the objects to a specified location.
We evaluate the policy by randomly choosing one of the distributions that corresponds to moving an object and plotting the final distance between the final object and its specified location.
We use the same GCRL baselines as before.
We also include two ablation: one that does not use the relabel the mean parameter $\mu$, which we label as \textbf{(-mean relabeling)}, and another that does not relabel the covariance parameter $\Sigma$, which we lavel as \textbf{(-cov relabeling)}.

We see in \autoref{fig:ablation-results} that relabeling all parameters of the distribution is necessary for fast learning.
In particular, without relabeling the mean parameter, the policy performs just as poorly as the GCRL baseline.

% \subsection{Task Specification with GDCRL}


% We present self-supervised in learning three domains which all exhibit difficulty in specifying the task as a goal state: box packing, ant navigation, and dexterous manipulation. All three are not naturally expressed as goal state reaching. In box packing the task is to put four objects into the box, without regard to where the objects are in the box. In ant navigation,
% the task is to move to a XY location, without regard to the joints of the robot. In dextrous manipulation, each task (door operning, object pickup, and nailing in a hammer) is defined by a small subset of the state variables. We show that our method can successfully learn in all of these environments through self-supervision.

% (Another good domain would be images)

% We compare against the following baselines, in order of importance:

% - exploration methods: goalgan, skewfit, discern

% - planning methods: SoRB, LEAP

% - "long horizon" methods?: reverse curriculum generation (but this uses reset to particular states)

% - hierarchical methods: HIRO, FuN, options, etc. (probably irrelevant)

% \subsection{Solving Long Horizon Tasks with GDCRL}

% In this experiment, we increase the number of objects in a box packing environment and demonstrate that our method is able to solve long-horizon tasks, while prior methods completely fail with more objects.

% \subsection{What Improves Exploration with GDCRL?}

% In this experiment, we investigate if it is higher quality data or a wider training distribution that improves performance.


\paragraph{Image-based distributions.}
We conduct preliminary image-based experiments on a two-dimension domain.
% As shown in \autoref{fig:2d-env-picture},
This environment comprises a blue circular cursor with radius $1.5$ which can move around in a 4-by-4 arena and two circular objects with radius $1$ that are randomly initialized in the scene.
The agent can interface with the cursor by specifying 2D velocity, and also a continuous grasp action between $-1$ and $1$.
When the grasp action non-negative, the agent will ``grab'' the nearest object within a small radius of its current location.
This object will move with the cursor until the agent releases the object by emitting a negative grasp action.
% The state contains the XY-position of the cursor and the objects.
The state is an image rendering of the scene, as show in \autoref{fig:2d-env-picture}.


==> draft/99_image_based_text.tex <==
from method (goal parameterization)

\paragraph{Nonlinear reparameterization.}
%%SL.7.10: My suggestion would be to define our method in a general way for *any* parametric distribution (not just Gaussians), and then have two "instantiation" subsections, one about how it can be instantiated with a Gaussian distribution, and one about how it be instantiated with arbitrary non-linear distributions via nonlinear reparameterization (which is this section). I don't think we should call it representation learning necessarily
%%GB.7.21: I agree with the above comment. 
There exist many tasks whose reward function cannot be written as \autoref{eq:mahalanobis-reward},
%%GB.7.21: But we said the above method can represent any reward function, now we are saying it does not? Also give an example.
and so we would like to develop a way to condition a policy on more expressive goal distribution families.
%%GB.7.21: What are more expressive families? Do you mean distributions that are not Gaussian distributions? It is not clear here.
% Normal distributions over the state space can only express rewards that that correspond to square Mahalanobis distances, but there are many tasks 
% Not all rewards can be expressed in terms of the log-likelihood of a normal distribution.
% Gaussians in the raw state space are limiting.
% One class of distribution
% To obtain more expressive distribution families, one can use neural networks to parameterize distributions~\citep{dinh2016density}.
One approach is to choose more expressive distribution families, such mixture models or distributions parameterized by neural networks~\citep{dinh2016density, van2016conditional}.
However, as the complexity of these models grows, so does the size of their parameter space.
% A variety of machine learning techniques, such as flow models, parameterize much more complex distributions using neural networks.
% However, conditioning a policy on the parameters of a neural network is impractical for most applications, 
In the extreme case, distributions based on neural networks often have millions of parameters~\citep{dinh2016density,kingma2018glow}.
% How can we express complex reward functions without needing to condition a policy on the weights of a neural network?
% but conditioning a policy on the parmeters of a neural network is hard.
%%GB.7.26: This should be earlier in the paper. The use of Gaussian distributions is already discussed.
%%SL.7.26: I edited the above paragraph, I think it's fine now

In order to obtain an expressive yet compact parameterization, we consider non-linear reparameterizations of the original state space.
Specifically, we model a distribution over the state space using a latent-variable model
\begin{align}\label{eq:non-linear-param}
    p_g(\bs; \omega) = \int_{\gZ} p_g(\bz ; \gdparam) p(\bs \mid \bz) d\bz,
\end{align}
where $p(\bs \mid \bz)$ is a generative model, and $p_g(\bz ; \gdparam)$ is a Gaussian distribution \emph{in a learned, latent space}.
% In other words, we can recover similar 
As we illustrate in \autoref{fig:representation-learning}
%%GB.7.26: A similar comment on this figure as in figure 1. This figure just shows that one can reparameterize a distirbution. It should be related to the method more. Can this be overlayed with image based task?
, the set of reward functions that can be expressed with \autoref{eq:non-linear-param} includes arbitrary non-linear transformations.
In the next section, we discuss how we acquire a latent space that is suitable for representing a desired set of tasks with normally distributed latent codes by using example data.

\begin{figure}
    \centering
    % \includegraphics[width=\linewidth]{figures/stub/representation_learning.jpg}
    \includegraphics[width=0.7\linewidth]{figures/contours/latent_to_complex_one.pdf}
    \caption{By learning a latent representation $z$ and a decoder $p(\bs \mid \bz)$, a simple Gaussian distribution in $\gZ$ space defines a complex distribution in the state space.}
    %%GB.7.21: Where did x come from? s has been used for state throughout the paper.
    \label{fig:representation-learning}
\end{figure}

From method (goal inference)

\paragraph{Non-Gaussian distributions.}

\begin{figure}
    \centering
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/stub/conditional_distribution.png}
        \caption{Conditional Distribution}
        \label{fig:my_label}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/stub/representation_learning_procedure.png}
        \caption{Latent Distribution}
        \label{fig:my_label}
    \end{subfigure}
    \caption{
    In addition to manually specifying distribution or using standard maximum likelihood estimation, we present two additional ways to learn distributions.
    (a) We construct a conditional distribution by learning a joint distribution over states where a subtask is completed and states where the complete task is completed. We then compute the resulting conditional distribution to dynamically construct distributions over states given a final task.
    (b) We construct a latent distribution that places high likelihood on states in $\dtask$ by mapping each state (left) into a posterior distribution over the latent space (center), and then fitting a single Gaussian distribution that minimizes KL-divergence to these distributions (right).}
    \label{fig:my_label}
\end{figure}

To represent more complex tasks, we would like to obtain a goal distribution of the form \autoref{eq:non-linear-param}, which defines a goal distribution $p_g(\bz; \gdparam)$ in a latent space $\gZ$.
We assume that we have access to $T$ states for learning a representation, which we denote as \mbox{$\drep = \{s_\text{rep}^{(t)}\}_{t=1}^T$},
as well as $K$ states in which a task is completed, which we denote as \mbox{$\dtask = \{s_\text{task}^{(k)}\}_{k=1}^K$}.
We note that the states used to train the representation $\drep$ do not need to be specific to a task since they are only used to learn the latent representation.

To embed states into a latent space where Gaussian distributions are meaningful, we use a Gaussian variational auto-encoder (VAE)~\citep{kingma2014vae,rezende2014stochasticbackprop}.
Gaussian VAEs models a set of observations, which in our case are states $\bs$, using a latent-variable model of the form
\begin{align*}
    p(\bs) = \int_{\gZ} p(\bz) p_\decparam(\bs \mid \bz) d\bz.
\end{align*}
The distribution $p_\decparam$ is a learned generative model or ``decoder'' and $p(z)$ is a standard multivariate Gaussian distribution in $\R^{d_z}$.
A Gaussian VAE also learns a posterior distribution or ``encoder'' that maps states $\bs$ onto Gaussian distributions in a latent space, given by $q_\encparam(\bz; \bs)$.
We refer readers to \citet{doersch2016tutorial} for a more thorough derivation, but in summary, a Gaussian VAE represents the distribution of all observations with standard Gaussian distribution in the latent space, given by $p(\bz)$, and represents a single observation $\bs$ with a Gaussian distribution in the latent space, given by $q_\encparam(\bz ; \bs)$.

\METHOD needs a Gaussian distribution that represents a task, as specified by a set of example states $\dtask$.
To obtain a distribution over the latent space that correspond to the task, we need a distribution in the latent space that places high likelihood on all of the states in $\dtask$.
We obtain such a distribution by finding a latent distribution that has minimum the KL divergence to the mixture of posteriors $\frac{1}{K} \sum_k q_\encparam(\cdot ; \bs_k)$.
Specifically, we solve the problem
\begin{align}\label{eq:latent-space-task-project}
    \gdparam* = \argmin_{\gdparam \in \gdspace} \DKL{
    \frac{1}{K} \sum_k q_\encparam(\bz ; \bs_k)
    }{p(\bz; \gdparam)},
\end{align}
where $\gdspace$ is the set of all means and diagonal covariance matrices in $\R^{d_z}$.
The solution to \autoref{eq:latent-space-task-project} can be computed in closed form using moment matching~\citep{minka2001expectation}.


==> draft/99_scrap.tex <==
We parameterize
Other bodies of work also study represe
Since we study how to train policies on a variety of tasks, our work is related 


Our method provides a way to learn policies that can accomplish a variety of different tasks, which is related to a variety of existing work on multi-task and meta-learning in reinforcement learning.
In meta-learning, a policy is trained to quickly adapt to new tasks, which may involve new dynamics ~\citep{nagabandi2018learning} or rewards~\citep{gupta2018meta,gupta18unsupervised,jabri2019unsupervised}, through interaction.
Rather than focusing on adapting to a new environment, we assume that tasks can be represented as sets of observations, allowing us to create a parametric representation of new tasks.
This parameterization allows us to perform zero-shot generalization rather than adaptation for new tasks, meaning that we do not need any additional test-time training.
Similarly, successor representations~\citep{dayan1993improving} and successor features~\citep{kulkarni2016deep,barreto2017successor,borsa2018universal,barreto2019transfer} assume a parametric form of reward functions in the form of weights to a linear feature space, but require that a user provides these features or supervision in the form of rewards rather than observations.

% We create a parametric 
% Meta-learning assumes tha
% meta-learning / multi-task learning
%  - difference: meta-learning methods don't assume that there's a parameterization to the task and so require inner-loop training
%      - \citep{teh2017distral}
%      - \citep{finn2017maml}
%      - \citep{xie2018few}
%      - \citep{nagabandi2018learning} (maml for adapting dynamics model)
%  - difference: we parameterize skills easily through sets to allow easy generalization
%      - parameterized skills (Da Silva et al., 2012)
%      - parameterized motor primitives (Kober et al., 2012)
%      - successor features  / GPI (require set of base features)
% goal distributions
%  - difference: they learn representation separately using VAE
%      - \citep{laversanne2018curiosity}

==> draft/old_notes.tex <==

\section{Problem}

How can we have a robot learn to assemble toys like \href{https://www.amazon.com/Take-Apart-Toys-Set-Construction/dp/B07392JXFR/ref=sr_1_14?keywords=toy+assembly&qid=1580474018&sr=8-14}{these}? The robot must compose a sequence of varied skills such as combining different pairs of parts, inserting a screw, or using a screwdriver. Acquiring the fine motor skills that can handle the variation in tasks and parts and develop robust controllers for each skill that adapt to errors in previous step will require collecting and learning from large amounts of data. A scalable solution requires little human overhead. How can we design a self-supervised system that can practice these separate skills and how to compose them by itself?

\subsection{Setting}

Consider a multi-step task with $N$ stages and a step reward $r(s, g) \in \{0, 1, \dots, N\}$. We start with an initial dataset $\gD = \{\gS_0, \gS_1, \dots, \gS_N,\}$ where $\gS_i$ is composed of state-goal tuples that satisfy $r(s, g) = i$. We will start with true state, but eventually want states and goals to be images.

This dataset may naturally be collected by labeling (demonstration) trajectories with rewards and considering the last observation as the goal. But it may be that collecting just the images is less cumbersome.

The aim is to recover a policy that maximizes $\E[\sum_t r(s, g)]$, although we never observe the true reward during training time after the initial dataset. (We can also consider settings where we do mostly self-supervised learning but intermittently get labeled rewards for the agent's trajectories.)

\section{Experiments}

We should set up a sequence of tasks with increasing difficulty to try to solve in this project.

\subsection{Tasks}
\textbf{Single-object pusher.} We have already solved single-object pusher to a reasonable degree, but there is still an issue where if you optimize reaching state goals, the algorithm must trade-off the hand reaching the hand goal position and the object reaching the object goal position. In reality, we only really care about the object position. Can we get better results by providing a sparse reward signal for the object goal?

\textbf{Multi-object pusher.} Similar to above but with multiple objects needing to be pushed to their goal locations. The reward could be +1 per object pushed to the correct location. (In the multi-step setting, the algorithm below should be modified to infer each task that provides a +1 reward.) This environment still needs to be defined; our Multiworld pusher supports inserting multiple objects but the workspace is not ideal for $>2$ objects. Michael J and Avi have been working on a PyBullet environment with many objects that might be relevant here.

\textbf{Multi-step assembly task.} To be defined.

\subsection{State vs. Vision}

Many of the issues we are considering are issues when learning from state, so I think we can work on all these ideas in state and then move to the RIG setting later on. This should not be too much more difficult as long as we use full state and avoid task-specific feature/reward engineering.

\section{Method}
\subsection{Notation}
% Consider a multi-step task with $N$ stages and a step reward $r(s, g) \in \{0, 1, \dots, N\}$. We start with an initial dataset $\gD = \{\gS_0, \gS_1, \dots, \gS_N,\}$ where $\gS_i$ is composed of state-goal tuples $o = (s, g)$ that satisfy $r(s, g) = i$. The set $\gS_{i \cdots j}$ denotes the union of $\{\gS_i \dots \gS_j\}$. For any tuple $o = (s, g)$, let $x = f(s, g)$, usually $x = s - g$.
Consider a multi-step task with $N$ stages. We start with an initial dataset $\gD = \{\tau_1, \tau_1, \dots, \tau_K\}$ where $\tau_i$ is composed of $N+1$ states that illustrate the waypoints to the goal $\{s_t^i\}$. At training and test time, we receive a goal state $g$ to reach.

\subsection{Practicing Skills with Goal Distributions}
In order to independently practice sub-skills of the entire task, we will infer a set of waypoint distributions $\{W_{ij}\}, W_{ij} \sim p_{\theta_{ij}} = \mathcal{N}(\mu_{ij}, \Sigma_{ij})$ corresponding to the achieving the specific sub-skill of stage $j$ while going from stage $i$ to the goal $g$ of the task.
%% GB.05.21.20: Does this imply that we will have to per-scribe the number of stages/goals need to solve the overall task? This is good for the start but it would be neet to bend this requirement.
%%AVN.05.22 Yes, for now I think we can just assume this but loosening this would be nice. One potential thing to consider is we have full demonstrations: can we learn waypoints that don't match exactly each timestep and are instead less granular?

For a particular waypoint $W$, the reward will be $r = \log p_W(s) = -||\Sigma^{-1/2}(s - \mu)||^2$ omitting irrelevant terms (this is the negative squared Mahalanobis distance). The policy and Q function will be conditioned on these parameters in order to generalize across them: $\pi(a|s, \theta)$ and $Q(s, a, \theta)$.
%% GB.05.21.20: It might be good to use a different variable (\phi maybe) to represent the goal distribution parameters.
At rollout time we can randomly sample $\theta_{ij}$ in order to collect coherent, meaningful samples. 
%% GB.05.21.20: While this is really an input to the models, including the Q function we could use gradient descent to optimize these parameters...
%%AVN.05.22 Could you explain a bit further? On what objective would be optimize $\theta$?
At test time, we could relabel with the same mixture distribution, or potentially consider a wider goal distribution.

We might fit these goal distributions directly to data, for instance by fitting the mean and covariance of examples from a particular stage. But for the tasks we are considering, the sub-goal distribution of interest is innately linked to the current state and final goal. To fit these waypoints, instead we should fit a density model to $p(s, w_{ij}, g)$ from the demonstrations, and then at rollout time infer $p(w_{ij}|s, g)$.

There are likely many choices for inferring $p(w_{ij}|s, g)$.
%% GB.05.21.20: Indeed. From demonstrations would be a good start. I think we can do more. 

\subsubsection{Gaussian Density}
To begin, we can fit a Gaussian $p(s_0, s_1, \dots, s_N)$. Then we will use $p(w_{ij}|s, g) = p(s_j|s_i, g)$ for inferring the mean and covariance.

The conditional distribution for a multivariate Gaussian $(X, Y)$ is given by 
\begin{align}
    \E[X|y] &= \mu_X + \Sigma_{XY} \Sigma^{-1}_{YY} (y - \mu_Y) \\
    \Cov[X|y] &= \Sigma_{XX} - \Sigma_{XY} \Sigma^{-1}_{YY} \Sigma_{YX}
\end{align}

This gives $\mu_{ij}, \Sigma_{ij}$ for the reward and policy conditioning.

\subsubsection{Gaussian Latent Density}
As above, but assume we are operating from high-dimensional observations or a low-dim observation where the tasks do not correspond to goal states (eg. move object 1 away from object 2). Then, learn a VAE on states such that the latent representation $p_\phi(z|s)$ satisfies $p(z_0, \dots, z_N) \sim \mathcal{N}$. You could do this by adding the objective $\min_{\theta,\phi} -\log p_\theta(z_1, \dots, z_N)$ to the VAE:
\begin{align}
    & l_k = (z_1, z_2, \dots, z_N)_k \\
    & \hat{\mu} = \E[L] \\
    & \hat{\Sigma} = \Cov[L] \\
    & \min_\phi \text{MSE}(\hat{\theta}).
\end{align}
That is, learn a representation $\phi$ so that a Gaussian fit to the waypoint dataset is a good fit. Perhaps some other choice of $D(L||\mathcal{N})$ that enforces $\{z_i\}$ being jointly Gaussian is better.

\subsubsection{Other Models}
We should consider how we would learn on higher dimensional tasks or on tasks where the feature space is not set up for the waypoint distribution to be linear in $s, g$. How could we learn features that are linear? Do we use a more complicated generative model, like a trajectory decoder? In that case, we might be limited by demonstration data - can we use the data we collect to learn that trajectory decoder online? Can we incorporate classifiers, like VICE does?

\subsection{Reward Learning as Classification}
For reward learning we will use classification, as in VICE. But instead of one classifier, we model two sets of classification problems:
\begin{align}
    L_i &= \1_{\{r = i\}} = \begin{cases} 
      l=0 & o \in S_i \\
      l=1 & o \in S_{i+1} \\
   \end{cases} \\
    H_i &= \1_{\{r \geq i\}} = \begin{cases} 
      h=0 & o \in S_{0 \dots i} \\
      h=1 & o \in S_{i+1 \dots N} \\
   \end{cases}
\end{align}
for $i \in {0, 1, \dots, N}$. The subtask random variable $L_i$ indicates the completeness of subtask $i$ and the cumulative task random variable $H_i$ indicates the completeness of the task up to $i$.

For any of these variables $Y_j$ we will obtain a reward by training a binary classifier on the corresponding sets.  We will choose reward functions that are something like:
\begin{align}
    r_{Y_j} = \log p_{Y_j} (y|x)
\end{align}
We will want to (severely) constrain the reward function in order to learn robust reward functions and in order to have parametric reward functions that we can optimize with a single parameter-conditioned policy and off-policy relabeling.

\subsection{Choice of Reward Function}
Different choices of the relationship between $Y_j$ and $X$ correspond to choosing different reward functions. Letting $Y_j \sim \text{Ber}(1/(1+\exp(-\theta_j^\T X)))$ and using:
\begin{align}
    r(s, g) &= \log \frac{p(Y_j=1|x)}{p(Y_j=0|x)} \\
            &= \theta_j^\T x.
\end{align}
So we simply use logistic regression to estimate $\theta_j$ and obtain the reward function. We could also estimate the distribution $p(\theta_j|\gD)$ instead of point estimates, which we could later use during RL. See section \ref{sec:infer_stochastic} for more details. Vitchyr suggests looking at looking at successor features for RL with this type of reward. Also, instead of $x=s-g$, augmenting $x = (s^2, g^2, s, g)$ would allow this to express norms.

We might also consider reward functions of the form:
\begin{align}
    r(s, g) &= -||M_t(s - g)|| \text{, where $M_t$ may be restricted to be diagonal or upper triangular} \\
    r(s, g) &= \1\{||M_t(s - g)|| \leq \epsilon\} \text{, where $\epsilon$ is also learned}
\end{align}
It's less clear to me how to estimate these properly but we could think more about it and heuristic solutions might just work. See section \ref{sec:infer_deterministic} for more details.

\subsection{Off-Policy RL}

The idea is that we treat $\{\theta_j\}$ as another thing we can sample for exploration and relabel off-policy while training, just like goals. We learn a policy $\pi(s, g, \theta)$ and action-value function $Q(s, g, \theta)$. When doing exploration, sampling various $\theta$ should allow us to do directed exploration for each subtask independently. But all data can be used to learn any of the subtasks due to off-policy relabeling. At test time, we evaluate $\theta_j$ corresponding to $H_{N-1}$.
%% GB.05.21.20: I am very interested in this idea. A type of HER that could help  the policy to understand its conditioning on the goal distributions better.

How to trade-off between subtasks ($L_i$) and cumulative tasks ($H_i$) could be an interesting question. For now, maybe we can just treat them uniformly. 

\section{Other Notes}
\subsection{Inferring the reward mask (deterministic)} \label{sec:infer_deterministic}
For each trajectory, consider training data for inferring the reward as $\{(s_t - g_t), R_t\}$. The data $(s_t - g_t)$ might look something like the below. 

\begin{center}
\begin{tikzpicture}
\begin{axis}[
    % title={Temperature dependence of CuSO$_4\cdot$5H$_2$O solubility},
    % xlabel={Temperature [\textcelsius]},
    % ylabel={Solubility [g per 100 g water]},
    xmin=-0.1, xmax=1,
    ymin=-0.1, ymax=1,
    xtick={0,1},
    ytick={0,1},
    legend pos=south east,
    ymajorgrids=false,
    % grid style=dashed,
]

\addplot[
    only marks,
    color=red,
    mark=x,
    ]
    coordinates {
    (0.3,0.5)(0.35,0.55)(0.4,0.7)(0.45,0.8)(0.55, 0.9)
    };
\addlegendentry{$R(s, g) = 0$}
    
\addplot[
    only marks,
    color=blue,
    mark=o,
    ]
    coordinates {
    (0.03,0.05)(0.1,0.1)(0.2,0.3)(0.15,0.2)(0.25,0.4)
    };
\addlegendentry{$R(s, g) = 1$}

\end{axis}
\end{tikzpicture}
\end{center}

Then the reward function $r(s, g)$ projects these points onto a scalar value parametrized by $m$. This is the core problem, and it would be great to come up with an elegant probabilistic model that suggests what the exact right structure for $R(s, g)$ and $r(s, g)$ is and how to infer $m$, where the relationship between $r$ and $R$ is something like $p(R=1|s,g) \propto \exp(r(s, g))$ (or some other distribution). This looks a lot like SVM/logistic regression. Figure out the right PGM is still to be done, but below is an ad-hoc method that will probably work.

The reward $r(s, g; m) = -||M(s - g)||$ parametrized by $m$ projects points onto a scalar value and we want to find a direction $\hat{m}$ that maximally separates these points. Let $x_t = s_t - g_t$ and $y_t = \begin{cases}
1, & R_t = 1\\
-1, & R_t = 0
\end{cases}$. Then we want $\hat{m}$ to maximally separate the points so let the loss function be
$$\max_{m, \mu} \; \sum_i (x_i \cdot \hat{m} - \mu)y_i$$
and learn $m$ through SGD. In practice the unit vector can be implemented by letting $m$ be all positive elements and $\hat{m} = m / \sqrt{m^\text{T}m + \epsilon}$. But this is just one suggestion.

\subsection{Inferring the reward mask (stochastic)} \label{sec:infer_stochastic}
Ideally, we would actually be able to track a distributions $p(m|\mathcal{D})$ over possible masks instead of computing the max likelihood one as above. 
At exploration time and at off-policy model training time we could then sample $m \sim p(m|\mathcal{D})$ similar to how we sample goals in HER/RIG. 
This should lead to coherent exploration of different possible reward functions.

One idea Sergey suggested is to infer $g = \mathcal{N}(\mu, \Sigma)$. Then $\log p(s = g) \alpha ||\Sigma^{-1} (s - g)|| $ ignoring irrelevant terms and assuming $\Sigma$ is diagonal. To have a distribution over $g$, Sergey suggested estimating an inverse Wishart as the distribution over $\Sigma$.

\textbf{Goal states.} In the case of only having a set of positive examples (eg. goal images along with robot states that satisfy the goal) then the above makes clear what we should do is just fit a multivariate Gaussian to that. This is the same as just considering the states where $R(s, g)=1$ but it feels like we should be able to use the negative information too. We should think about the connection between this and goal-conditioned VICE.

\subsection{Why Constrain Reward Functions} \label{sec:constrain}
The two key challenges in reinforcement learning are unknown dynamics, and unknown reward functions. By disentangling these problems and addressing them separately, we can come up with efficient algorithms. This suggests a hierarchical RL algorithm with two levels: the lower level one understands how to handle unknown dynamics, and the higher level one handles the unknown reward function.

The lower level one that handles unknown dynamics has been the topic of a lot of prior work and could be done in many forms. The most obvious one is learning a dynamics model, as in model-based RL, but the same can be achieved implicitly by learning a policy to reach states as in goal-conditioned RL or even supervised learning of inverse dynamics models. In this work we will consider goal-conditioned RL.

The higher level one to handle unknown reward functions is less studied and the one we will focus on in this work. 
Reward functions have a lot of structure - they are often some sort of distance between observation features. Separating out the reward function inference will allow us to take advantage of the structure: we will consider inferring contextual reward functions of the form $r_M(s, g) = -||M(s - g)||$, where $M$ is an unknown matrix/mask. 
We could infer the reward from demonstrations, sparse rewards, or preferences. 
In the following we will focus on inferring from a sparse reward function because it is a convenient way for humans to supervise the learning process, but keep in mind there are other options. 
This structure (along with an algorithm to take advantage of it) should allow the agent to practice the specific task we care about, and practice subsets of tasks in multi-step hierarchical tasks.

\section{Old Introductions}

\section{Introduction (V1)}

%% More general motivation for method and problem
We want
%%SL.6.25: seems a bit informal
robots to be intelligent problem solvers.
While reinforcement learning
can enable agents to autonomously learn policies that maximize reward on a task, it
%%SL.6.25: a bit informal
has struggled with finding solutions to long horizon problems.
%%GB.6.24: We could start to talk about the compsitional nature of tasks here.
Being capable of solving tasks that involve many steps is a hallmark of general intelligence,
%%SL.6.25: Some AI researchers and many robotics researchers will have an aversion to papers that use the term "general intelligence," to the point of reflexively rejecting them.
it implies the agent has learned a good representation and can explore to solve new tasks.   
%%SL.6.25: This feels a bit backwards, and I'm not really sure in what direction this is going. I think what you are trying to get at is that learning representations and exploring is important to solve multi-step tasks, but this point is not really made clearly in the above sentence.
%%GB.06.24: Should expand on this more.
Long horizon planning tasks particularly difficult for robotics applications that do not have the luxury of fast or cheap data.
How can a robot automatically expand its skills and grow its ability to solve increasingly long tasks?
%%SL.6.25: The above paragraph is too unfocused and disjointed. Try to make sure that each sentence follows logically from the previous one (at the lower level), and at the higher level, try to clearly motivate the main idea in the work. I would strongly recommend rereading the paper writing guide, especially the section of the guide that pertains to introductions.

% Most long-horizon problems present very hard exploration problems. However, most practical long-horizon problems can be decomposed into shorter sub-tasks that users semantically understand. We can make learning easier by providing semantic demonstration for each sub-task. 
% important to emphasize the focus on observation-only demonstrations
% We also want to talk about how we want demonstrations that complete tasks in different orders.
%% We want to search in the space of plans now, not just goals.
Most long-horizon problems present very hard
%%SL.6.25: too informal
exploration problems. However, most practical long-horizon problems can be decomposed into shorter sub-tasks that users
%%SL.6.25: somewhat jarring shift in focus -- why are we talking about users all of a sudden?
semantically understand.
%%GB.06.24: What do we mean by semantically understand?
This decomposition is key,
%%SL.6.25: key for what?
as it leads to reducing the problem from learning the full long horizon problem to learning how to connect portions or sub-tasks together via sub-goals. 
%%GB.06.24: This sentence is a bit confusing.
In contrast to recent self-supervised methods for goal exploration,
%%SL.6.25: which ones? and why are we contrasting to them?
we instead want
%%SL.6.25: too informal
to additionally explore in the space of plans.
%%SL.6.25: I don't think this makes sense. In what way are we exploring in the space of plans?
We want
%%SL.6.25: too informal
a method that does not need to explore all $k^{n}$ plans,
%%SL.6.25: the level of detail in this sentence will make the reader think that "plans" has been formally defined, and leave them frustrated to realize that it hasn't
where $k$ is the number of sub-tasks and $n$ is the plan length, in order to solve them if asked to. Instead, given the provided sub-goal structure, the robot may only need to reach from a goal to all other goals, requiring only $k^2$ pairs. This greatly reduces the number of \textit{tasks} the robot needs to learn how to solve. Still it is tricky to learn this task decomposition without additional information.
%% Need a better connection sentence.
%%SL.6.25: There is a very jarring and sharp shift in the level of detail in the above paragraph. The first half is too high level, the second half too high level. Motivate your choices before stating them clearly.

%% 
% We can make learning easier by providing semantic demonstration for each sub-task. 

%% While learning from demonstration has been shown to improve learning this is not really the type of structure we want to learn. We don't just want a method that can repeat an expert, we want machine learning methods that discover the underlying task structure and be able to use this knowledge to make learning/planning easier.
%%GB.6.24: We want to discuss how learning this goal distribution give us a new method for the exploration of sub-tasks or plans.
While learning from demonstration has been shown to improve learning
%%SL.6.25: repetitive
this may not be the type of structure we want to learn from demonstration data. We don't want
%%SL.6.25: too informal
a method that can repeat an expert, we want
%%SL.6.25: too informal
machine learning methods that discover the underlying task structure and be able to use this knowledge to make learning/planning easier.
In this work, rather than learning to directly imitate,
%%SL.6.25: the discussion of imitation kind of comes out of nowhere
we instead learn a \textit{semantic} decomposition of the task space to increase reuse. This is accomplished by learning a goal proposal distribution from a small collection of demonstrations without actions. These goal proposal distributions are then used to provide a form of sub-task exploration.
%%GB.6.24: Explain more why this is important. It does not seem clear enough yet to the reader.
Each sub-task is shorter and easier to solve than the original tasks using common goal condition reinforcement learning methods. Using this system tasks can now be specified at test time as a sequence of sub-goals by a human or via another learning process. 

%% Why without actions?


%% Our main contribution is a method to decompose and explore an a goal subspace learned from a few task demonstrations. Using this method we are able to solve tasks that involve many more steps than typical RL methods.
Our main contribution is a method to decompose and explore a goal subspace learned from a few task demonstrations. Using this method we are able to solve tasks that involve many more steps than typical RL methods. We are also able to solve long plans for which demonstrations were not provided. This shows that the robot is able to learn how to generalize in the form of connecting and re-ordering sub-task between demonstrations.

\section{Introduction (V2)}
% Many real-world robot problems often require long-horizon control.
% How can we to train robots to accomplish complex tasks while minimizing the amount of engineering burden and training time?
% Reinforcement learning provides an appealing formalism for robots to acquire various skills, but users need to balance the amount of supervision they provide with the amount of time needed for these robots need to learn.
% Learning-based approaches are appealing, but they require users to balance 
% Learning-based approaches often str
An open problem in robot learning is striking a balance between minimizing supervision cost and training time.
For example, training a robot to accomplish a complex task, such as assembling furniture, by only providing a sparse reward does not require much input from a user, but most learning systems will struggle to find a solution in a reasonable amount of time without any supervision from the user.
%%SL.6.25: I think focusing the contribution on supervision from the user is a mistake. There is a lot of depth in how to design user interfaces, and that's not really what this paper is about.
%%GB.6.26: This will also motivate the comparison to more supervised learning methods. Which we don't want.
Most of these complex problems can be divided into smaller problems, such as pick-and-place tasks, each of which can be solved by learning based systems.
%%GB.6.26: What is a learning based system? While I might understand your point, we can use this opportunity to instead inform the reader with more details related to the problem.
However, if users need to manually design rewards or provide extensive supervision (e.g., expert demonstrations) for each individual task, the engineering burden can quickly out-weigh the benefits of using these learning systems.
We instead want a method in which users can easily decompose complex tasks into smaller tasks, without needing extensive engineering for each new task.
%%GB.6.26: Most of this can be made better by removing the dependance on "users" and demonstration. We chatted about this yesturday so I think it is known how this would change.

% by only providing a sparse reward at the end of training might eventually work, but exploration would probably be too difficult.
% Fortunately, many practical robot problems can be decomposed into tasks, each of which can be solved in a tractable amount of time.
% Many of these problems can be decomposed into sub-tasks, each of which can be easier to solve
% On one hand
% However, manually designing rewards for each task requires a lot of engineering (e.g. manually designing rewards), then this would defeat the whole point of having a learning-based agent.

A cheap source of supervision is to convey each task through \textit{example sets}.
For example, rather than writing a reward function to tell a robot to move an object to a location, a user can provide example observations of what it looks like to move an object to a certain location.
%%GB.6.26: While I like the example sets idea I don't think a minimal user input view is the right motivation for this.
% Rather than designing a new reward function or providing demonstrations, a user can provide a set of example observations of what it looks like to move an object to a certain location.
% To address these concerns, we consider the problem of learning to solve tasks that are conveyed through example sets.
% Sets are appealing because they convey the semantics of a task (e.g. goals over-specify problems), and are relatively easy to provide (e.g. you don’t need actions).
These example sets can be significantly easier to provide than demonstrations, since they do not require action demonstrations.
Moreover, they do not need to specify how a task is solve (e.g. the exact sequence of states needed), but rather only need to what the task looks like upon completion.

While providing example sets for different tasks may be simple, training a separate policy for each task is time-consuming and does not exploit potential shared structure between different tasks. For example, the representations learned to screw an object into a hole is likely similar to the representations needed to insert a peg into a hole.
Moreover, training separate policies for each task does not provide a mechanism for generalizing to new tasks: given a new task, we would need to train an entirely new policy.

To exploit shared structure between the tasks and allow generalization, we propose to train a policy that is conditioned on the example set.
In other words, rather than training a different policy for each different task, we give the example observations to the policy.
However, unlike similar work, such as goal-conditioned reinforcement learning, there’s an inherent ambiguity that we need to address:
given an example set, the task is not to reach one of those states exactly.
Instead, the agent needs to understand that these observations are only representatives of some more general task.

In order to represent tasks, we use the example sets to learn a distribution over the state space.
We then condition a policy on the parameters to this distribution, which we also use to compute the rewards.
Given a new example set, we extract a distribution of the state space, give the distribution parameters to our policy, and can perform zero-shot testing…


% Given a set of example observations, we train a 
% In practice, it’s not that we want to give rewards only when a state is the example set is reached.
% What we actually want to 
% In practice, the example set isn’t completely exhaustive--it’s only a representative subset.
% We represent sets using distributions over the state space.

Our main contribution is a method called TBD that allows us to train set-conditioned policies in a sample-efficient manner.
We demonstrate that TBD allows us to solve multiple tasks in parallel that share data.
Overall, we demonstrate that we can then use TBD and cheap example sets to solve long-horizon robot control problems.

\section{Introduction (V3) - focused on exploration}

% Learning and composing skills for long horizon assembly tasks

In the future, we will expect to robots to be able to compose sequences of varied skills such as combining pairs of parts for an assembly task, or using a screwdriver to insert a screw. 
Acquiring the fine motor skills that can handle the variation in tasks and parts and develop robust controllers for each skill that adapt to errors in previous step will require collecting and learning from large amounts of data.
A scalable solution to collecting large amounts of manipulation data requires little human overhead. 
How can we design a self-supervised system that can practice these separate skills autonomously and how to compose them to perform multi-step tasks?

% % What is the problem: self-supervised learning with long horizon tasks
% Deep learning excels at generalizing from very large datasets.
% %%GB.6.26:I don't think this is true. 
% While deep reinforcement learning has been applied succesfully to robotics tasks in recent years, the required supervision cost of real-world robotics has prevented us from working in the very large data regime in robotics. 
% %%GB.6.26: It is not clear what the large data regime is? More spcifics could help make this more clear.
% To get there, we need methods that can autonomously learn behaviors with little human involvement. 
% Goal-conditioned reinforcement learning is a promising approach towards self-supervised RL: by using simple and general reward functions for goal-reaching, goal conditioned RL allows agents to supervise their own learning without manually engineered reward functions. But without human-shaped reward functions, the RL problem becomes more and more difficult as the learning horizon increases, especially when solving complex multi-step tasks.
% %%GB.6.26: There is still too much focus on needing input from the user. Maybe we can take a bit of a skew-fit approach and discuss more about goal exploration distributions and why they are important.

Goal-conditioned reinforcement learning is a promising approach towards self-supervised RL: by using simple and general reward functions for goal-reaching, goal conditioned RL allows agents to supervise their own learning from raw observations without manually engineered reward functions. 
% If we were able to solve long-horizon tasks with self-supervised learning, we could instead learn a diverse array of tasks by specifying a final goal image. 
%%GB.6.26:This connection is not clear enough to the reader. I am not even sure how to connect these easily. More description of the self-supervised method could help make this connection more clear. However, we should only go into detail on this if this is view we want to use to explain the method.
Goal-conditioned RL has been applied to learn manipulation skills from raw observations such as images~\cite{nair2018rig}.
This could enable the learning of complex manipulation tasks from a goal image.
For instance, a robot could learn to assemble a newly designed motherboard by attempting to insert each part according to the image of the fully assembled board. 
%%GB.6.26: These two sentences seem to be unrelated
% More broadly, such a system could collect vast amounts of data on various tasks, and enable generalization in robotic manipulation.
But without human-shaped reward functions, the RL problem very difficult as the learning horizon increases, especially when solving complex multi-step tasks.

% % Why is it interesting and important: we could solve a range of tasks with little supervision
% If we were able to solve long-horizon tasks with self-supervised learning, we could instead learn a diverse array of tasks by specifying a final goal image. 
% %%GB.6.26:This connection is not clear enough to the reader. I am not even sure how to connect these easily. More description of the self-supervised method could help make this connection more clear. However, we should only go into detail on this if this is view we want to use to explain the method.
% Imagine in an industrial setting, a robot could learn to assemble a newly designed motherboard by attempting to insert each part according to the image of the fully assembled board. 
% %%GB.6.26: These two sentences seem to be unrelated
% More broadly, such a system could collect vast amounts of data on various tasks, and enable generalization in robotic manipulation.
% %%GB.6.26: While this is a nice message it needs more introduction to lead to this conclusion. From this I see why it could me important but more detail is needed to understand why it is interesting.

% Why is it hard
The main difficulty is exploration: collecting meaningful data, particularly without the guidance of human reward shaping. General reward functions, such as state distance, can be too sparse or poorly shaped to learn from for difficult multi-step tasks. Prior methods to perform long horizon tasks without reward shaping have required demonstrations and large amounts of exploration data. Providing demonstrations is burdensome and also scales poorly due to the combinatorial explosion of possible sequences of skills.
Moreover, reaching a particular goal state is not general enough: we may instead want to communicate a set of potential subgoals that could assist in exploration and better describe the task.
How can we enable better exploration with little additional supervision?
%%GB.6.26: This paragraph starts out well but by the end it feels like the difficulty is how to provide better demonstrations. This is a bit a minefield of an area to motivate the method from.

% Your method
The key to better exploration in long-horizon tasks is understanding sub-tasks and performing them coherently. To this end, we propose to improve exploration by extending goal-conditioned RL to learn sub-tasks. We introduce goal-distribution conditioned RL, in which tasks and sub-tasks are represented as goal-distributions. These goal distributions are inferred from a small set of examples, and probability of the state under a goal distribution induces a natural reward function. The policy is conditioned on the parameters of the distribution, allowing for meaningful exploration in the absence of supervision and thereby successful policy execution for very long-horizon tasks.
%%GB.6.26: This sounds better. It is a bit disconnected from the previous paragraph and would benifit from a little more detail, for example, what is a goal distribution? How does it enable meaningful exploration?

% Contributions of this paper
The main contribution of this paper is to introduce goal-distribution conditioned RL and its application to the self-supervised learning of long-horizon tasks. We demonstrate that we can solve multi-step assembly tasks using this method, without an extrinsic reward signal.

\section{Introduction (V4)}

% Learning and composing skills for long horizon assembly tasks

In the future, we will expect to robots to be able to compose sequences of varied skills such as combining pairs of parts for an assembly task, or using different screwdrivers to insert different screws. 
Acquiring the fine motor skills that can handle the variation in tasks and parts and develop robust controllers for each skill that adapt to errors in previous step will require collecting and learning from large amounts of data.
A scalable solution to collecting large amounts of manipulation data requires minimal human overhead. 
%%GB.06.28: This sentence lacks clarity. Is something scalable as long as people don't have to be involved? This just makes it more automated, not that it will improve with more data or less human oversight.
How can we design a self-supervised system that can practice these separate skills autonomously and how to compose them to perform multi-step tasks?
%%GB.06.28: This is a good start. The paragraph needs more details to ease the reader into the motivation more. For example, what is "self-supervised" learning and why is it a good thing?

% % What is the problem: self-supervised learning with long horizon tasks
% Deep learning excels at generalizing from very large datasets.
% %%GB.6.26:I don't think this is true. 
% While deep reinforcement learning has been applied succesfully to robotics tasks in recent years, the required supervision cost of real-world robotics has prevented us from working in the very large data regime in robotics. 
% %%GB.6.26: It is not clear what the large data regime is? More spcifics could help make this more clear.
% To get there, we need methods that can autonomously learn behaviors with little human involvement. 
% Goal-conditioned reinforcement learning is a promising approach towards self-supervised RL: by using simple and general reward functions for goal-reaching, goal conditioned RL allows agents to supervise their own learning without manually engineered reward functions. But without human-shaped reward functions, the RL problem becomes more and more difficult as the learning horizon increases, especially when solving complex multi-step tasks.
% %%GB.6.26: There is still too much focus on needing input from the user. Maybe we can take a bit of a skew-fit approach and discuss more about goal exploration distributions and why they are important.

% % Why is it interesting and important: we could solve a range of tasks with little supervision
Goal-conditioned reinforcement learning is a promising approach towards self-supervised RL: by using simple and general reward functions for goal-reaching, goal conditioned RL allows agents to supervise their own learning from raw observations without manually engineered reward functions. 
% If we were able to solve long-horizon tasks with self-supervised learning, we could instead learn a diverse array of tasks by specifying a final goal image. 
%%GB.6.26:This connection is not clear enough to the reader. I am not even sure how to connect these easily. More description of the self-supervised method could help make this connection more clear. However, we should only go into detail on this if this is view we want to use to explain the method.
Goal-conditioned RL has been applied to learn manipulation skills from raw observations such as images~\cite{nair2018rig}.
These methods enable the learning of complex manipulation tasks specified by a goal image.
%%GB.06.28: This sentence is a little repetitive from the previous sentence. Also, what is "this"?
For instance, a robot could learn to assemble a newly designed motherboard by attempting to insert each part according to the image of the fully assembled board. 
%%GB.06.28: This paragraph is also a good start. I think is requires the reader to know a far bit about GCRL. As it is a now, a goal is just some term in the clouds that is not grounded enough for the reader to see a clear picture. Add a sentence to explain what an example of a goal is, this will also help the reader understand what goals are in the next paragraph. 

% Why is it hard
But this approach suffers from two issues as we apply it to more general tasks. 
%%GB.06.28: What is a more general task? It would be good to conceptualize the problem a little more to allow the reader to understand this over-specification more. 
First, goal-conditioned reinforcement learning relies on task specification with a goal state, which may over-specify the task. Reaching a particular goal state is not general enough: we may instead want to communicate a set of potential outcomes such as two objects being attached, or focus on a subset of the state space such as the position of an object without regard to other state variables.
%%GB.06.28: More details for this example would be good. It would be great if it connected back to the example at the beginning of this introduction.
Second, without human-shaped reward functions, the RL problem is very difficult as the learning horizon increases, especially when solving complex multi-step tasks.
The main difficulty is exploration: collecting meaningful data, particularly without the guidance of human reward shaping.
%%GB.06.28: It is not clear how these two sentences connect, one is about exploration and the next is about reward functions. Tell the reader how do reward functions fix/affect exploration? Something along the lines of how bad reward functions provide misleading signal and good ones instead encourage the agent to explore that state space...
General reward functions, such as state distance, can be too sparse or poorly shaped to learn from for difficult multi-step tasks.

% Your method
We propose a new framework, goal-distribution conditioned reinforcement learning, to address both issues. 
%%GB.06.28: I thought we were calling the method set-conditioned?
Tasks are represented as goal-distributions , instead of points, which are inferred from a small set of examples.
Goal distributions are expressive, capturing a large family of tasks, and induces a natural reward function.
%%GB.06.28: While this may be true this sentence needs to be unpacked. We need to smack the reader in the face why point goals can't do somethings that are important and using goal distributions allow us to do new things (or things properly). Each of the points in this sentence need there own sentence to explain why they are important. If not here then earlier in the intro.
The policy is conditioned on the parameters of the distribution, allowing for zero-shot generalization and efficient learning through relabeling.
%%GB.06.28: Why does this conditioning on the parameters allow for those things? I think this part of the paper really needs a diagram to clearly explain the problem.
Additionally, sub-task examples can also be provided and used to infer additional goal distributions.
%%GB.06.28: What is a sub-task example? What happened to goals and how are they connected to tasks?
The key to better exploration in long-horizon tasks is understanding sub-tasks and performing them coherently; inferring subgoals allows the agent to practice the sub-tasks meaningfully during exploration even when it 
%%GB.06.28: What is "it"?
does not solve the full task early on in training.
%%GB.06.28: I don't know if agree with this sentence. However, we don't need to re motivate the method here. We should have more details and connect those choices back to the motivation from the previous paragraphs.

% Contributions of this paper
The main contribution of this paper is to introduce goal-distribution conditioned RL and its application to the self-supervised learning of long-horizon tasks. We demonstrate that we can solve multi-step assembly tasks using this method, without an extrinsic reward signal.


==> tmp.tex <==

\subsection{Dynamics Constraints \tmp{Still in the air if this is to be included}}
To better shape the latent space and take advantage of the temporal consistency of trajectories, we enforce dynamics constraints. We evaluate the following three architectures following \cite{watter2015embed}:
\begin{enumerate}
    \item Global linear dynamics:
        % $$z_{t+1} = A \begin{bmatrix} z_t \\ u_t \end{bmatrix}$$
        $$\hat{z}_{t+1} = A z_t + B u_t$$
    \item Locally linear dynamics:
        $$\hat{z}_{t+1} = f_{\theta_1}(z_t, u_t) z_t + g_{\theta_2}(z_t, u_t) u_t$$
    \item Neural network dynamics:
        $$\hat{z}_{t+1} = f_\theta(z_t, u_t)$$
\end{enumerate}
We assume a Gaussian output distribution, so these constraints are enforced through a L2 loss: $\mathcal L_\text{dyn} = ||\hat{z}_{t+1} - z_{t+1}||^2$. 



\subsection{Adversarial Learning for Disentangled Representations \tmp{Not using - probably deleting}}

Although the optimal solution of the model specified above should not pass information about $s_0$ through the latent variable $z$, empirically we find that the optimization does not always find this optimum solution. This entangling of the representation causes issues during RIG. To actively disentangle $s_0$ and $z$ we additionally minimize $I(z; s_0)$ in our training objective.

To do this, following [also cite Barber+Agakov] \cite{chen2016infogan} we introduce another decoder $Q$ and observe that:
\begin{align}
    I(z; s_0) &= H(s_0) + \E_{z} \E_{s_0 \sim P(s_0|z)} [\log P(s_0|z)] \\
    &= H(s_0) + \E_{z} \E_{s_0 \sim P(s_0|z)} [\log Q(s_0|z) +  \\ & \hspace{2cm} D_\text{KL}( P(.|z) || Q(.|z) ] \\
    &\geq H(s_0) + \E_{z} \E_{s_0 \sim P(s_0|z)} [\log Q(s_0|z)] \\ 
    &= \mathcal L_\text{I}
\end{align}

We parametrize the $Q$ and train it to maximize $L_\text{I}$, which amounts to maximizing the log-likelihood of reconstructing $s_0$ from $z$, while the encoder minimizes the full objective:
\begin{align} \label{eq:isc-vae-loss-adv}
    \mathcal L = \E_{q_\phi(z|s, s_0)} [\log p(s|z, s_0)] - \beta D_{KL}(q_\phi(z|s, s_0)||p(s)) + \mathcal L_\text{I}
\end{align}


\begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=1\linewidth]{img/pointmass1_reward_curve.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \center
        \includegraphics[width=1\linewidth]{img/pusher1_reward_curve.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=1\linewidth]{img/reward_curve_avg_cloth.png}
    \end{subfigure}
    \caption{Visualization of distance in latent space to last state in a trajectory - different representation learning methods.}
    \label{fig:reward-curves}
\end{figure}


%%%% ABSTRACT COMMENTS:
% To allow robots to perform useful tasks in unconstrained settings,
% To allow robots to act in the wild,
%%SL.1.20: kind of sounds like you want them to put on a play during a safari
% they must be able to handle significant task and object diversity. 
% Reinforcement learning (RL) may enable this by allowing robots to autonomously learn from data.
% However, we face several challenges towards general robot learning in collecting interaction data that captures meaningful tasks, and providing supervision to the robot to learn useful skills. 
%%SL.6.22: A suggestion for phrasing here could be something like this: 
In order to create skilled robots that can perform a variety of manipulation skills in a wide range of real-world situations, with complex inputs such as images, they must learn behaviors that generalize effectively over rich and diverse datasets. To enable such a data-driven approach to scale, the robot must be able to collect its own experience without reliance on human labeling and supervision -- only then can such a method generalize broadly and effectively.
% The supervision cost of RL has not been appreciated fully: RL requires a ground truth reward signal, and most RL algorithms assume an episodic setting of the problem with environment resets.
%%SL.1.20: The episodic thing I think is something many people will object to... while it may be true, I think it's not obvious to many people that it is true.
% Both are significant challenges in the real world. 
% Second, to allow a robot to learn a variety of skills with different objects, the agent must be able to successfully explore skills with each object, and understand how to reuse these skills.
%%SL.1.20: I think you'll get some argument as to whether "skill" is in fact the right word here
% We investigate self-supervised learning to handle these challenges, and show that we can autonomously learn skills, such as pushing and grasping of various objects through interaction using goal-conditioned RL.
% Using model-free learning, we are able to take advantage of large datasets to learn these skills in a sample efficient, off-policy manner.
%%SL.6.22: Potential rephrasing here could go something like this: 
Scalable robotic learning without supervision is difficult, the robot needs to be able to set its own goals to practice diverse skills, and incorporate large off-policy datasets into its learning process. 
%%AVN.7.4 seems to assume goal-conditioned framework before introducing it
%%SL.7.5: I think that's OK -- the "without supervision -> set its own goals" progression seems OK. I'm a bit more concerned about how, if we back off on the off policy training story, the datasets part might be no longer true.
In this paper, we study how such a method can be instantiated for a real-world robotic system. Our method bootstraps off of a large off-policy dataset, and then uses autonomous interaction via a conditional goal proposal model to gather additional goal-directed experience. The conditional goal proposal model sets goals -- by generating image-based states -- that are feasible to reach in the current environment, while still being diverse enough to provide for useful skill learning and data collection. Our experiments show that such an approach learns policies that can achieve a wide variety of visually indicated goals at test time, including reaching, pushing, and grasping of diverse objects.
%%SL.7.5: Perhaps if we end up having to cut the off-policy/data-driven story, we could go with something like this. Maybe you could also borrow parts of this to rewrite the intro if we go with that story.
% While reinforcement learning provides an appealing formalism for learning individual skills, a truly general-purpose robotic system must be able to master a large repertoire of behaviors. Instead of learning a large collection of skills individually, can we instead enable a robot to propose and practice its own behaviors automatically, learning about the affordances and behaviors that it can perform in its environment, such that it can then repurpose this knowledge once a new task is commanded by the user? In this paper, we study this question in the context of self-supervised goal-conditioned reinforcement learning. A central challenge in this learning regime is the problem of goal setting: in order to practice useful skills, the robot must be able to autonomously set goals that are feasible but diverse. When the robot's environment and available objects vary, as they do in most open-world settings, the robot must propose to itself only those goals that it can actually accomplish in its present setting with the objects that are at hand. Previous work only studies self-supervised goal-conditioned RL in single-environment settings, where goal proposals from the robot's past experience or from a generative model are sufficient. In more diverse settings, this frequently leads to impossible goals and, as we show experimentally, prevents effective learning. We propose a conditional goal-setting model that aims to only propose goals that are feasible reachable from the robot's current state, and demonstrate that this enables self-supervised goal-conditioned learning with raw image observations both in varied simulated environments and a real-world cloth manipulation task.


% Samples from 

% For a particular environment, a dataset of 100 trajectories of length 100 with random actions is constructed and 10\% of the trajectories are set aside as the test set.
% %%SL.7.1: It's better to use active voice. Also, what does "for a particular environment" mean? Which environment? Maybe fine if you're testing on all, but if it's one specific one, better to just say it.
% Given a test trajectory, $\{s_0, s_1, ..., s_T\}$, the reconstruction of image $s_t$ is created by first computing $q_\phi(z|s_t, s_0)$, sampling $z \sim q_\psi(s|z, s_0)$, and computing $q_\psi(s|z, s_0)$. Samples are drawn for this trajectory by sampling $z \sim N(0, I)$ and generating image $q_\psi(s|z, s_0)$.
%%SL.7.1: Discuss results? How do we measure/evaluate if they're good? What is the conclusion to be drawn from this?

% \subsection{Context-Conditioned VAE Metric}
% %%SL.7.1: One thing that makes me uneasy about this section is how it contributes to the overall message in the paper. Are we claiming that something about our contribution makes this better (vs prior work)? If so, can we present evidence of this?

% In this experiment, we consider the distance metric induced by the learned encoder of our model. This is vital to use for RIG,
% %%SL.7.1: Is it *actually* vital? It's not actually obvious (at least not to me).
% as RIG uses the reward function $$r_t = ||z_t - z_g||.$$

% %%SL.7.1: I think the paragraph below could be rearranged to put more of the rationale (what are you trying to evaluate?) first, and then the method, otherwise it first states the method (what you measure) and then the rationale (what are you trying to determine by measuring this)
% To visualize the reward function for different methods, we consider a set of trajectories of optimal policies. For each trajectory $\{s_0, s_1, ... s_H \}$, we consider the distance $||\phi(z_t) - \phi(z_H)||$ for each value of $t$. We average these distances over the trajectories and report the average per timestep for each feature embedding $\phi$. Smoothly decreasing distances indicate a smooth latent space and a favorable dense reward signal, while a flat curve that sharply decreases near the final timestep indicates a poorly shaped latent space that will require RL to handle a sparse reward signal.

